A Framework for Approximation Schemes on Disk Graphs

We initiate a systematic study of approximation schemes for fundamental optimization problems on disk graphs, a common generalization of both planar graphs and unit-disk graphs. Our main contribution is a general framework for designing efficient polynomial-time approximation schemes (EPTASes) for vertex-deletion problems on disk graphs, which results in EPTASes for many problems including Vertex Cover, Feedback Vertex Set, Small Cycle Hitting (in particular, Triangle Hitting), $P_k$-Hitting for $k\in\{3,4,5\}$, Path Deletion, Pathwidth $1$-Deletion, Component Order Connectivity, Bounded Degree Deletion, Pseudoforest Deletion, Finite-Type Component Deletion, etc. All EPTASes obtained using our framework are robust in the sense that they do not require a realization of the input graph. To the best of our knowledge, prior to this work, the only problems known to admit (E)PTASes on disk graphs are Maximum Clique, Independent Set, Dominating set, and Vertex Cover, among which the existing PTAS [Erlebach et al., SICOMP'05] and EPTAS [Leeuwen, SWAT'06] for Vertex Cover require a realization of the input disk graph (while ours does not). The core of our framework is a reduction for a broad class of (approximation) vertex-deletion problems from (general) disk graphs to disk graphs of bounded local radius, which is a new invariant of disk graphs introduced in this work. Disk graphs of bounded local radius can be viewed as a mild generalization of planar graphs, which preserves certain nice properties of planar graphs. Specifically, we prove that disk graphs of bounded local radius admit the Excluded Grid Minor property and have locally bounded treewidth. This allows existing techniques for designing approximation schemes on planar graphs (e.g., bidimensionality and Baker's technique) to be directly applied to disk graphs of bounded local radius.

==> OLD/Saket/preamble-more.tex <==
%\newtheorem{theorem}{Theorem}[section]
\newtheorem{remark}{Remark}




==> OLD/Saket/preamble-short.tex <==
%Color and Pictures
\usepackage[usenames,svgnames]{xcolor}
\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{decorations.shapes}


%Formatting and Layout
\usepackage{wrapfig}
%\usepackage{fullpage}
\usepackage{xspace}

%Pretty boxes
\usepackage{framed}
\usepackage{boxedminipage}


%Math
\usepackage{amsmath,amssymb}
\usepackage[retainorgcmds]{IEEEtrantools}
\usepackage{pdfpages}
\usepackage{lastpage}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{multicol}
\renewcommand{\thefootnote}{\Roman{footnote}}


% Eat up the page numbers: 
%\pagenumbering{gobble}


%Multiple Author Names & Affiliations
\usepackage{authblk}


%Linked References 
%%%\usepackage[pagebackref,linktocpage]{hyperref}
\usepackage{hyperref}

\hypersetup{
    pdfauthor={Neeldhara Misra},     % author
    pdfnewwindow=true,      % links in new window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=SlateBlue,          % color of internal links
    citecolor=FireBrick,        % color of links to bibliography
    filecolor=magenta,      % color of file links
    urlcolor=Emerald           % color of external links
}

%A useful package if you write url addresses:
\usepackage{url}


% Dutch style of paragraph formatting, i.e. no indents. 
%\setlength{\parskip}{1.3ex plus 0.2ex minus 0.2ex}
%\setlength{\parindent}{0pt}





%Macros

\newcommand{\FPT}{\textrm{\textup{FPT}}\xspace}
\newcommand{\WOH}{\textrm{\textup{W[1]-hard}}\xspace}
\newcommand{\WTH}{\textrm{\textup{W[2]-hard}}\xspace}
\newcommand{\NP}{\textrm{\textup{NP}}\xspace}
\newcommand{\NPH}{\textrm{\textup{NP-hard}}\xspace}
\newcommand{\NPC}{\textrm{\textup{NP-complete}}\xspace}

\newcommand{\OO}{{\mathcal O}}
\newcommand{\name}[1]{\textsc{#1}}
\newcommand{\YES}{\textsc{Yes}}
\newcommand{\NO}{\textsc{No}}

\newcommand{\problembox}[4]{
\begin{framed}
{\bf #1} \hfill Parameter: {#3} \\
\begin{tabular}{p{.15\textwidth} p{.8\textwidth}}
% | p{.25\textwidth} p{.7\textwidth} | 
%\hline
\hfill Input: & {#2}\\
%\hfill Parameter: & {#3}\\
\hfill Question: & {#4}\\
%\hline
\end{tabular}
\end{framed}
}




==> OLD/Saket/preamble.tex <==
%Color and Pictures
\usepackage[usenames,svgnames]{xcolor}
\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{decorations.shapes}

%Formatting and Layout
%\usepackage{wrapfig}
%\usepackage{titlesec}
%\usepackage{titling}
%\usepackage{fullpage}
\usepackage[margin=1in,nohead]{geometry}
%%\usepackage{xspace}
%\usepackage[ruled,noline,linesnumbered]{algorithm2e}
%\usepackage{multicol}
%%Pretty boxes
%\usepackage{framed}
\usepackage{boxedminipage}
\usepackage{stmaryrd}

%Math

\usepackage{amsmath,amssymb,amsthm}

\usepackage[retainorgcmds]{IEEEtrantools}
\usepackage{pdfpages}
\usepackage{lastpage}

\usepackage{enumerate}
%Fonts!
%\usepackage{ifxetex}
%
%\ifxetex
%      \usepackage{fontspec}
%      \usepackage{xunicode}
%      \defaultfontfeatures{Mapping=tex-text} % To support LaTeX quoting style
%      \usepackage{euler}
%      \usepackage[small,euler-digits]{eulervm}
%      \newfontfamily\specialfont{Merge Light}
%      %Set formats for each heading level
%    \titleformat*{\section}{\Large\bfseries\sffamily\color{SlateGray}\specialfont}
%    \titleformat*{\subsection}{\large\bfseries\sffamily\color{DimGray}\specialfont}
%    \titleformat*{\subsubsection}{\itshape\specialfont}
%    \renewcommand{\maketitlehooka}{\specialfont}
%    \newfontfamily\fancyheading{Lorena}
%    \newcommand\cuteheading[1]{{\fancyheading #1}}
%    
%    
%    %%%%%%\setromanfont{Baramond}
%    \setromanfont[SmallCapsFont={Overlock SC}]{Overlock}
%    
%    
%\else
%  \usepackage[utf8]{inputenc}
%  \usepackage[T1]{fontenc}
%\fi
%\renewcommand{\thefootnote}{\Roman{footnote}}


% Eat up the page numbers: 
%\pagenumbering{gobble}


%Multiple Author Names & Affiliations
\usepackage{authblk}

%Clever References
%\usepackage{cleveref}
%\usepackage[backend=bibtex]{biblatex}
%\bibliography{backdoorstw,references}
%
%
%\AtEveryBibitem{% Clean up the bibtex rather than editing it
% \clearlist{address}
% \clearfield{date}
% \clearfield{eprint}
% \clearfield{isbn}
% \clearfield{issn}
% \clearlist{location}
% \clearfield{month}
% \clearfield{series}
% \clearfield{url} 
% \ifentrytype{book}{}{% Remove publisher and editor except for books
%  \clearlist{publisher}
%  \clearname{editor}
% }
%}

%Linked References 
%%%\usepackage[pagebackref,linktocpage]{hyperref}
%\usepackage{hyperref}
\usepackage{booktabs}
\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = SlateBlue,
                 urlcolor  = blue,
                 citecolor = FireBrick,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref}

%\hypersetup{
%    pdfauthor={Neeldhara Misra},     % author
%    pdfnewwindow=true,      % links in new window
%    colorlinks=true,       % false: boxed links; true: colored links
%    linkcolor=SlateBlue,          % color of internal links
%    citecolor=FireBrick,        % color of links to bibliography
%    filecolor=magenta,      % color of file links
%    urlcolor=Emerald           % color of external links
%}

%A useful package if you write url addresses:
\usepackage{url}


% Dutch style of paragraph formatting, i.e. no indents. 
%\setlength{\parskip}{1.3ex plus 0.2ex minus 0.2ex}
%\setlength{\parindent}{0pt}


%ToDo Notes
\usepackage[backgroundcolor=Moccasin,colorinlistoftodos]{todonotes}

\makeatletter
 \providecommand\@dotsep{5}
 \def\listtodoname{}
 \def\listoftodos{\@starttoc{tdo}\listtodoname}
 \makeatother

\newcommand{\addref}{\todo[color=MistyRose]{Ref!}}

% Author specific comment commands

\newcounter{nmcomment}
\newcommand{\nmtodo}[1]{%
    % initials of the author (optional) + note in the margin
    \refstepcounter{nmcomment}%
    {%
        \todo[color={LightSteelBlue},size=\small,inline]{%
            \textbf{Comment [NM\thenmcomment ]:}~#1}%
}}




%Macros

\newcommand{\FPT}{\textrm{\textup{FPT}}\xspace}
\newcommand{\WOH}{\textrm{\textup{W[1]-hard}}\xspace}
\newcommand{\WTH}{\textrm{\textup{W[2]-hard}}\xspace}
%\newcommand{\NP}{\textrm{\textup{NP}}\xspace}
\newcommand{\NPH}{\textrm{\textup{NP-hard}}\xspace}
\newcommand{\NPC}{\textrm{\textup{NP-complete}}\xspace}

\DeclareMathOperator{\poly}{poly}
\newcommand{\Ptime}{{\ensuremath{\rm{P}}}}
\newcommand{\NP}{{\ensuremath{\rm{NP}}}}
\newcommand{\coNP}{{\ensuremath{\rm{coNP}}}}

\newcommand{\name}[1]{\textsc{#1}}
\newcommand{\YES}{\textsc{Yes}}
\newcommand{\NO}{\textsc{No}}
\newcommand{\FAIL}{\textsc{Fail}}

\newcommand{\problembox}[4]{
\begin{framed}
{\sc #1} \hfill Parameter: {#3} \\
\begin{tabular}{p{.15\textwidth} p{.8\textwidth}}
% | p{.25\textwidth} p{.7\textwidth} | 
%\hline
\hfill Input: & {#2}\\
%\hfill Parameter: & {#3}\\
\hfill Question: & {#4}\\
%\hline
\end{tabular}
\end{framed}
}


\newcommand{\defparproblem}[4]{
 % \vspace{1mm}
\begin{tcolorbox}[colback=gray!10!white,colframe=gray!75!black]
% \begin{minipage}{.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
 % \end{minipage}
\end{tcolorbox}
  %\vspace{1mm}
}

\newcommand{\defproblem}[3]{
  %\vspace{1mm}
\begin{tcolorbox}[colback=gray!5!white,colframe=gray!75!black]
 % \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1   \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  %\end{minipage}
  \end{tcolorbox}
 % \vspace{1mm}
}


%\newcommand{\defparproblem}[4]{
%  \vspace{3mm}
%\noindent\fbox{
%  \begin{minipage}{.95\textwidth}
%  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} \textsc{#1}  & {\bf{Parameter:}} #3 \\ \end{tabular*}
%  {\bf{Input:}} #2  \\
%  {\bf{Question:}} #4
%  \end{minipage}
%  }
%  \vspace{2mm}
%}
%
%\newcommand{\defproblem}[3]{
%  \vspace{3mm}
%\noindent\fbox{
%  \begin{minipage}{.95\textwidth}
%  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  \\ \end{tabular*}
%  {\bf{Input:}} #2  \\
%  {\bf{Question:}} #3
%  \end{minipage}
%  }
%  \vspace{2mm}
%  }


\newcommand{\AAA}{{\mathcal A}}
\newcommand{\BB}{{\mathcal B}}
\newcommand{\CC}{{\mathcal C}}
\newcommand{\DD}{{\mathcal D}}
\newcommand{\EE}{{\mathcal E}}
\newcommand{\FF}{{\mathcal F}}
\newcommand{\GG}{{\mathcal G}}
\newcommand{\HH}{{\mathcal H}}
\newcommand{\II}{{\mathcal I}}
\newcommand{\JJ}{{\mathcal J}}
\newcommand{\KK}{{\mathcal K}}
\newcommand{\LL}{{\mathcal L}}
\newcommand{\MM}{{\mathcal M}}
\newcommand{\NN}{{\mathcal N}}
\newcommand{\OO}{{\mathcal O}}
\newcommand{\PP}{{\mathcal P}}
\newcommand{\QQ}{{\mathcal Q}}
\newcommand{\RR}{{\mathcal R}}
\newcommand{\SSS}{{\mathcal S}}
\newcommand{\TT}{{\mathcal T}}
\newcommand{\UU}{{\mathcal U}}
\newcommand{\VV}{{\mathcal V}}
\newcommand{\WW}{{\mathcal W}}
\newcommand{\XX}{{\mathcal X}}
\newcommand{\YY}{{\mathcal Y}}
\newcommand{\ZZ}{{\mathcal Z}}

\newcommand{\aaa}{{\mathfrak a}}
\newcommand{\bbb}{{\mathfrak b}}
\newcommand{\ccc}{{\mathfrak c}}
\newcommand{\ddd}{{\mathfrak d}}
\newcommand{\eee}{{\mathfrak e}}
\newcommand{\fff}{{\mathfrak f}}
%\newcommand{\ggg}{{\mathfrak g}}
%\newcommand{\hhh}{{\mathfrak h}}
\newcommand{\iii}{{\mathfrak i}}
\newcommand{\jjj}{{\mathfrak j}}
\newcommand{\kkk}{{\mathfrak k}}
%\newcommand{\lll}{{\mathfrak l}}
\newcommand{\mmm}{{\mathfrak m}}
\newcommand{\nnn}{{\mathfrak n}}
\newcommand{\ooo}{{\mathfrak o}}
\newcommand{\ppp}{{\mathfrak p}}
\newcommand{\qqq}{{\mathfrak q}}
\newcommand{\rrr}{{\mathfrak r}}
\newcommand{\sss}{{\mathfrak s}}
\newcommand{\ttt}{{\mathfrak t}}
\newcommand{\uuu}{{\mathfrak u}}
\newcommand{\vvv}{{\mathfrak v}}
\newcommand{\www}{{\mathfrak w}}
\newcommand{\xxx}{{\mathfrak x}}
\newcommand{\yyy}{{\mathfrak y}}
\newcommand{\zzz}{{\mathfrak z}}


\newcommand{\ol}[1]{\overline{#1}}

% Paper specific macros.

\newcommand{\mtext}[1]{\text{\normalfont #1}}
\newcommand{\pp}{\mtext{ppar}}

\newcommand{\lcac}[1]{{\mbox{\bf LCA-closure}(#1)}}
\newcommand{\forget}{\mbox{\bf forget}}

\newcommand{\rp}{$r$-protrusion}
\newcommand{\rpp}{$r'$-protrusion}
\newcommand{\pmin}{{\sc min-CMSO}}
\newcommand{\peq}{{\sc $p$-eq-CMSO}}
\newcommand{\pmax}{{\sc max-CMSO}}
\newcommand{\pmem}{{\sc $p$-min/eq/max-CMSO}}
\newcommand{\pmm}{{\sc $p$-min/max-CMSO}}
\newcommand{\pem}{{\sc $p$-eq/max-CMSO}}
\newcommand{\pmeq}{{\sc $p$-min/eq-CMSO}}

\newcommand{\inc}{{\normalfont \textsf{inc}}}
\newcommand{\tw}{{\normalfont \textsf{tw}}}
\renewcommand{\sb}{{\normalfont \textsf{sb}}}
\newcommand{\wb}{{\normalfont \textsf{wb}}}

\newcommand{\var}{{\normalfont \textsf{var}}}
\newcommand{\cla}{{\normalfont \textsf{cla}}}
\newcommand{\lit}{{\normalfont \textsf{lit}}}

\renewcommand{\restriction}{\mathord{\upharpoonright}}
\newcommand{\wbtw}{{\textsc{$\WW_t$-Weak Backdoors}}}

\newcommand{\satgraph}{SAT incidence graph}
\newcommand{\satgraphs}{SAT incidence graphs}


\newcommand{\ig}{incidence graph}
\newcommand{\igs}{incidence graphs}

%\newcommand{\bigoh}{\ensuremath{\OO}}
\newcommand{\al}{\Sigma}
\newcommand{\OR}{{\ensuremath{\rm{OR}}}}
\newcommand{\AND}{{\ensuremath{\rm{AND}}}}

\newcommand{\prel}{\mathcal{R}}
\newcommand{\pequiv}{\equiv_{\prel}}


\newcommand{\nats}{{\ensuremath{\mathbb{N}}}}
\newcommand{\ints}{{\ensuremath{\mathbb{Z}}}}
\newcommand{\identity}{{\ensuremath{\mathrm{id}}}}
\newcommand{\compass}{\NP\subseteq \coNP/\poly}
\newcommand{\ncompass}{\NP\nsubseteq \coNP/\poly}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\samplingsizethreshold}[3]{{\sf samp_sz}(#1,#2,#3)}
\newcommand{\samplingtreewidththreshold}[3]{\tau(#1,#2,#3)}
\newcommand{\recundsizethreshold}[3]{\rho_{\sf sz}(#1,#2,#3)}
\newcommand{\successprobability}[3]{p(#1,#2,#3)}



\newcommand{\tweta}[0]{{\rm tw}-$\eta$ {\rm CNF}}

\newcommand{\teta}[0]{$\eta$-tw}


\newcommand{\what}{\widehat}
\newcommand{\wtilde}{\widetilde}


\newcommand{\gridminorbound}[1]{\ensuremath{#1^{100}}}



\newcommand{\leaf}[1]{{\sf leaf}(#1)}

% Paper specific macros.


\newcommand{\Yes}{\textsf{yes}}
\newcommand{\No}{\textsf{no}}

\newcommand{\chsfull}{\textsc{Conn. $\cH$-HS}}
\newcommand{\coNPbypoly}{${\sf co\- NP/Poly}$}
%\newtheorem{redr}[theorem]{Reduction Rule}



\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cF}{{\mathcal{F}}}

\newcommand{\X}{{\mathcal{X}}}

\newcommand{\GETS}{\ensuremath{\leftarrow}}
\newcommand{\TO}   {{\bf to }}
\newcommand{\STEP}  {{\bf step }}
%\newcommand{\AND} {{\bf and }}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cI}{\mathcal{I}}
%\newcommand{\cP}{\mathcal{P}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cB}{\mathcal{B}}

\newcommand{\cD}{\mathcal{D}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cK}{\mathcal{K}}
%\newcommand{\cP}{\mathcal{P}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\algo}[1]{\texttt{#1}}
\newcommand{\prob}[1]{\mathrm{Prob}[~#1~]}
\newcommand{\mean}[1]{\mathrm{\bf E}[~#1~]}
\newcommand{\Zplus}{\Z^+}
%\newcommand{\Rplus}{{\cal R}^+}
%\newcommand{\Rplus}{{\cal R}^{\geq}}
\newcommand{\OPT}{\mbox{\rm OPT}}
\newcommand{\LP}{\mbox{\rm LP}}
\newcommand{\DLP}{\mbox{\rm D-LP}}
%\newcommand{\D}{{\cal D}}
\newcommand{\CTHS}{\mbox{\rm C$\diamondsuit$HS}}
\newcommand{\CFVS}{\mbox{\rm CFVS}}
\newcommand{\CPFD}{\mbox{\rm CP$\cF$D}}
\newcommand{\typzero}{{\sf Type 0}}

\newcommand{\typone}{{\sf Type 1}}
\newcommand{\typtwo}{{\sf Type 2}}
\newcommand{\taip}[1]{{\sf Type #1}}


\newcommand{\eps}{\varepsilon}
%\newcommand{\prob}[1]{{\it #1}}
%\newcommand{\prob}[1]{\textit{#1}}
%\newcommand{\algo}[1]{{\sc #1}}
\newcommand{\I}{\mathcal{I}}
%\newcommand{\DD}{\mathcal{D}}
\newcommand{\eS}{\mathcal{S}}
\newcommand{\K}{\mathcal{K}}
%\newcommand{\PP}{\mathcal{P}}
%\newcommand{\C}{\mathcal{C}}
\newcommand{\B}{\mathcal{B}}
%\newcommand{\G}{\mathcal{G}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\eL}{\mathcal{L}}
\newcommand{\pr}{\mathbf{Pr}}
%%
\newcommand{\R}{\mathbb{R}}


\newcommand{\no}{{\sc NO}}


%\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}{Claim}[section]
%\newtheorem{corollary}{Corollary}
%\newtheorem{definition}{Definition}[section]
%\newtheorem{observation}{Observation}[section]
\newtheorem{proposition}{Proposition}[section]
\newcounter{reduction}
\setcounter{reduction}{0}
\newcounter{markingrule}

\setcounter{markingrule}{0}
\newtheorem{mschm}[markingrule]{Marking Scheme}
\newtheorem{redr}[reduction]{Reduction Rule}
\newtheorem{marule}[markingrule]{Marking Rule}
\newcommand{\cJ}{{\mathcal J}}


%\newcommand{{\red}}[1]{\fbox{\textcolor{red}{#1}}}
%\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1} \ }}
%\newcommand{\mypara}[1]{\smallskip\noindent{\textbf{\sffamily #1} \ }}

\newcommand{\hcovering}[0]{$k$-{\sc $\cH$-covering}}
\newcommand{\hpacking}[0]{{\sc $\cH$-packing}}

%
%\newcommand{\compass}{\NP\subseteq \coNP/\poly}
%\newcommand{\ncompass}{\NP\nsubseteq \coNP/\poly}

\renewcommand*\overline[1]{%
%
%\newcommand*\oline[1]{%
   \vbox{%
     \hrule height 0.5pt%                  % Line above with certain width
     \kern0.25ex%                          % Distance between line and content
     \hbox{%
       \kern-0.15em%                        % Distance between content and left side of box, negative values for lines shorter than content
       \ifmmode#1\else\ensuremath{#1}\fi%  % The content, typeset in dependence of mode
       \kern-0.1em%                        % Distance between content and left side of box, negative values for lines shorter than content
     }% end of hbox
   }% end of vbox
}

\usetikzlibrary{shapes.geometric,matrix,shapes,arrows,positioning,chains}




\newenvironment{problemOPT}[2][]{\noindent\ignorespaces%
                                \FrameSep=6pt%
                                \parindent=0pt%
                \vspace*{-.5em}
                \ifthenelse{\isempty{#1}}{%
                  \begin{GrayBox}{\textsc{#2}}%                
                }{%
%                  \begin{GrayBox}{\textsc{#2} parameterized by~{}}%  
                }
                \newcommand\Prob{{\sf Feas. sol.:}}%
                \newcommand\Input{{\sf Input:}}%
                \newcommand\Parameter{{\sf Parameter:} }          
                \begin{tabular*}{\textwidth}{@{\hspace{.1em}} >{\itshape} p{1.2cm} p{0.85\textwidth} @{}}%     
            }{
                \end{tabular*}%
                \end{GrayBox}%
                \vspace*{-.5em}
                \ignorespacesafterend
            } 
            
            

\newcommand{\msrTodo}[1]{\todo[inline]{#1}}
\newcommand{\specSccFtransversal}[0]{{\sc Strict SCC $\cF$-Transversal}}
\newcommand{\sccFTransversal}[0]{{\sc SCC $\cF$-Transversal}}
\newcommand{\SOPT}[0]{S_{\sf OPT}}
            
            
            
             \newcommand{\relevant}[0]{{\sf rel}}
                          \newcommand{\connectors}[0]{{\sf conn}}

\newcommand{\algsfvs}[0]{\textsf{Alg{-}Disjoint{-}SFVS}}
\newcommand{\algcompressionsfvs}[0]{\textsf{Alg{-}Compression{-}SFVS}}

 \newcommand{\strictalgsfvs}[0]{\textsf{Alg{-}Strict{-}SFVS}}
 \newcommand{\strictalgdoct}[0]{\textsf{Alg{-}Strict{-}DOCT}}

            \newcommand{\algdoct}[0]{\textsf{Alg{-}Disjoint{-}DOCT}}

            \newcommand{\algsbimc}[0]{\textsf{Alg{-}Disjoint{-}BiMC}}
 \newcommand{\strictalgsbimc}[0]{\textsf{Alg{-}Strict{-}BiMC}}
 
 \newcommand{\mN}[0]{{\mathbb N}}
\newcommand{\mO}[0]{{O}}
\newcommand{\mR}[0]{{\mathbb R}}
\newcommand{\mA}[0]{{\mathbb A}}
\newcommand{\sol}{{\rm sol}}
\newcommand{\cost}{{\rm cost}}
\newcommand{\goal}{{\rm goal}}
\newcommand{\maximum}{{\rm max}}
\newcommand{\minimum}{{\rm min}}
\newcommand{\opt}{{\rm opt}}


 


==> OLD/Saket/saketPreamble.tex <==
%\usepackage{microtype}%if unwanted, comment out or use option "draft"
\usepackage{wrapfig}
\usepackage{bm}

\usepackage{xspace}
\newcommand{\pname}{\textsc}
\newcommand{\ProblemFormat}[1]{\pname{#1}}
\newcommand{\ProblemIndex}[1]{\index{problem!\ProblemFormat{#1}}}
\newcommand{\ProblemName}[1]{\ProblemFormat{#1}\ProblemIndex{#1}{}\xspace}

\newcommand{\probPVD}{\ProblemName{Planar Vertex Deletion}}
\newcommand{\probCVD}{\ProblemName{Chordal Vertex Deletion}}
\newcommand{\probEB}{\ProblemName{Edge Bipartization}}
\newcommand{\probOCT}{\ProblemName{Odd Cycle Transversal}}
\newcommand{\probEMC}{\ProblemName{Edge Multiway Cut}}
\newcommand{\probVMC}{\ProblemName{Vertex Multiway Cut}}
\newcommand{\probGFVS}{\ProblemName{Group Feedback Vertex Set}}
\newcommand{\probGFES}{\ProblemName{Group Feedback Edge Set}}
\newcommand{\probEMultiC}{\ProblemName{Edge Multicut}}
\newcommand{\probVMultiC}{\ProblemName{Vertex Multicut}}
\newcommand{\probSFVS}{\ProblemName{Subset Feedback Vertex Set}}

\newcommand{\probTWdel}{\ProblemName{Treewidth-$\eta$ Modulator}}
\newcommand{\probFdel}{\ProblemName{$\mathcal{F}$-Deletion}}
\newcommand{\probFpack}{\ProblemName{$\mathcal{F}$-Packing}}
\newcommand{\probSdel}{\ProblemName{$\mathcal{S}$-Deletion}}
\newcommand{\probSpack}{\ProblemName{$\mathcal{S}$-Packing}}
% Commonly used names
\newcommand{\probVC}{\ProblemName{Vertex Cover}}
\newcommand{\probPlVC}{\ProblemName{Planar Vertex Cover}}
\newcommand{\probPVC}{\ProblemName{Partial Vertex Cover}}
\newcommand{\probPDS}{\ProblemName{Partial Dominating Set}}
\newcommand{\probPrDS}{\ProblemName{Partial $r$-Dominating Set}}
\newcommand{\probFVS}{\ProblemName{Feedback Vertex Set}}
\newcommand{\probIFVS}{\ProblemName{Independent Feedback Vertex Set}}
\newcommand{\probCycPacking}{\ProblemName{Cycle Packing}}
\newcommand{\probPlFVS}{\ProblemName{Planar Feedback Vertex Set}}
\newcommand{\probIS}{\ProblemName{Independent Set}}
\newcommand{\probWIS}{\ProblemName{Weighted Independent Set}}
\newcommand{\probMCIS}{\ProblemName{Multicolored Independent Set}}
\newcommand{\probDS}{\ProblemName{Dominating Set}}
\newcommand{\probrDS}{\ProblemName{$r$-Dominating Set}}
\newcommand{\probrSC}{\ProblemName{$r$-Scattered Set}}
%\newcommand{\probMDS}{\ProblemName{Minimum Dominating Set}}
\newcommand{\probPlDS}{\ProblemName{Planar Dominating Set}}
\newcommand{\probCDS}{\ProblemName{Connected Dominating Set}}
\newcommand{\probDST}{\ProblemName{Dominating Set on Tournaments}}
\newcommand{\probClique}{\ProblemName{Clique}}
\newcommand{\probMC}{\ProblemName{Multicolored Clique}}
\newcommand{\probPClique}{\ProblemName{Partitioned Clique}}
\newcommand{\probqSC}{\ProblemName{$q$-Set Cover}}
\newcommand{\probSC}{\ProblemName{Set Cover}}
\newcommand{\probDSP}{\ProblemName{Dominating Set with Pattern}}
%\newcommand{\probOCT}{\ProblemName{Odd Cycle Transversal}}
%\newcommand{\probEB}{\ProblemName{Edge Bipartization}}
\newcommand{\probHam}{\ProblemName{Hamiltonian Cycle}}
\newcommand{\probPlHam}{\ProblemName{Planar Hamiltonian Cycle}}
\newcommand{\probHamP}{\ProblemName{Hamiltonian Path}}
\newcommand{\probKPath}{\ProblemName{Longest Path}}
\newcommand{\probWKPath}{\ProblemName{Weighted Longest Path}}
\newcommand{\probthreeSAT}{\ProblemName{$3$-SAT}}
\newcommand{\probqSAT}{\ProblemName{$q$-SAT}}
\newcommand{\probcnfSAT}{\ProblemName{CNF-SAT}}
\newcommand{\probthreeCol}{\ProblemName{$3$-Coloring}}
\newcommand{\probqCol}{\ProblemName{$q$-Coloring}}
\newcommand{\probListColoring}{\ProblemName{List Coloring}}
\newcommand{\probOddSet}{\ProblemName{Odd Set}}
\newcommand{\probTuring}{\ProblemName{Short Turing Machine Acceptance}}
\newcommand{\probSI}{\ProblemName{Subgraph Isomorphism}}
\newcommand{\probGI}{\ProblemName{Graph Isomorphism}}
\newcommand{\probWCS}{\ProblemName{Weighted Circuit Satisfiability}}
\newcommand{\probClosestString}{\ProblemName{Closest String}}
\newcommand{\probClosestSubstring}{\ProblemName{Closest Substring}}
\newcommand{\probGridTiling}{\ProblemName{Grid Tiling}}
\newcommand{\probGridTilingLeq}{\ProblemName{Grid Tiling with~$\le$}}
\newcommand{\probUnitDisk}{\ProblemName{Unit Disk Independent Set}}
\newcommand{\probEMWay}{\ProblemName{Edge Multiway Cut}}
\newcommand{\probEDS}{\ProblemName{Edge Dominating Set}}
\newcommand{\probEMWaySets}{\ProblemName{Edge Multiway Cut for Sets}}
\newcommand{\probDirEMWay}{\ProblemName{Directed Edge Multiway Cut}}
\newcommand{\probEMCut}{\ProblemName{Edge Multicut}}
\newcommand{\probMulticut}{\ProblemName{Multicut}}
\newcommand{\probDirEMCut}{\ProblemName{Directed Edge Multicut}}
\newcommand{\probSkewEMCut}{\ProblemName{Skew Edge Multicut}}
\newcommand{\probDFVS}{\ProblemName{Directed Feedback Vertex Set}}
\newcommand{\probDFAS}{\ProblemName{Directed Feedback Arc Set}}
\newcommand{\probDFASC}{\ProblemName{Directed Feedback Arc Set Compression}}
\newcommand{\probPartpq}{\ProblemName{$(p,q)$-Partition}}
\newcommand{\probClusterpq}{\ProblemName{$(p,q)$-Cluster}}
\newcommand{\probSatellite}{\ProblemName{Satellite Problem}}
\newcommand{\probTw}{\ProblemName{Treewidth}}
\newcommand{\probPerfSetMatch}{\ProblemName{Perfect $d$-Set Matching}}
\newcommand{\probHS}{\ProblemName{Hitting Set}}
\newcommand{\probdHS}{\ProblemName{$d$-Hitting Set}}
\newcommand{\probEdHS}{\ProblemName{E$d$-Hitting Set}}
\newcommand{\probSetSplit}{\ProblemName{Set Splitting}}
\newcommand{\probSteiner}{\ProblemName{Steiner Tree}}
\newcommand{\probSteinerF}{\ProblemName{Steiner Forest}}
\newcommand{\probMotif}{\ProblemName{Graph Motif}}
\newcommand{\probColorfulMotif}{\ProblemName{Colorful Graph Motif}}
\newcommand{\probRBDSlong}{\ProblemName{Red-Blue Dominating Set}}
\newcommand{\probRBDS}{\ProblemNameX{RBDS}{Red-Blue Dominating Set}}
\newcommand{\probCRBDSlong}{\ProblemName{Colored Red-Blue Dominating Set}}
\newcommand{\probCRBDS}{\ProblemNameX{Col-RBDS}{Colored Red-Blue Dominating Set}}
\newcommand{\probCVC}{\ProblemName{Connected Vertex Cover}}
\newcommand{\probCFVS}{\ProblemName{Connected Feedback Vertex Set}}
\newcommand{\probCBullHit}{\ProblemName{Connected Bull Hitting}}
\newcommand{\probSetPacking}{\ProblemName{Set Packing}}
\newcommand{\probDisFactors}{\ProblemName{Disjoint Factors}}
\newcommand{\probDisPaths}{\ProblemName{Vertex Disjoint Paths}}
\newcommand{\probChromatic}{\ProblemName{Chromatic Number}}
\newcommand{\probECC}{\ProblemName{Edge Clique Cover}}
\newcommand{\probSubsetSum}{\ProblemName{Subset Sum}}
\newcommand{\probKnapsack}{\ProblemName{Knapsack}}
\newcommand{\probWayCut}{\ProblemName{$s$-Way Cut}}
\newcommand{\probEulerian}{\ProblemName{Eulerian  Deletion}}
\newcommand{\probBisec}{\ProblemName{Minimum Bisection}}
\newcommand{\probMaxBisec}{\ProblemName{Maximum Bisection}}


==> Saket/applications.tex <==
In this section, we apply our framework of Section \ref{sec:framework} on several problems to obtain sub-exponential algorithms on $H$-minor free graphs. Given the framework, its application on a problem is fairly straightforward, except we have to ensure that the problem satisfies the requirements of this framework. First, we apply this framework on \probOCT and describe all the steps in detail. For other problems, the applications are similar. Thus, for convenience, we will just describe the changes needed for those problems omitting the trivial details. In all of our problems, we assume that the input graph is $H$-minor-free. 

\subsection{\probOCT and \probEB}
First, we consider the  \probOCT (OCT) problem. In OCT, we are given a graph $G=(V,E)$ and a parameter $k$, and we would like to decide whether there is a subset $V'\subseteq V$ of size at most $k$ such that for each odd cycle $C$ in $G$, there is a vertex of $C$ that is in $V'$. If there is such a subset, we refer to it as a solution. By abusing the notation, we refer to a solution to the OCT problem also as an OCT. The distinction should be clear from the context. Following our framework, the first step is to apply Lemma~\ref{lem-candidate} to obtain a candidate set $\mathsf{Cand} \subseteq V$ for the instance. Note that this takes only a polynomial time. For our purpose, it is sufficient to find a solution which is a subset of $\mathsf{Cand}$. Henceforth, by the term solution we always mean a subset of $\mathsf{Cand}$.       

Note that after removing the vertices in an OCT from $G$, a bipartite graph is left. For such a bipartition, we arbitrarily define the left and the right side (or partition). Consider any subgraph $G_1=(V_1,E_1)$ and fix any solution to OCT on $G_1$. We define a configuration $\lambda$ of $V'\subseteq V_1$ w.r.t. the solution to be a set of values corresponding to the vertices  in $V'$, where each value is in $\{1,2,3\}$. We note that these three values denote whether the corresponding vertex $v$ is in the solution, is in the left side of the residual bipartite graph (after removing the solution OCT) or is in the right side of the residual bipartite graph. As we want our solution to be a subset of $\mathsf{Cand}$, the 1-vertices must always come from $\mathsf{Cand}$. Otherwise, we say the configuration is not valid. 

\subsubsection{Contraction-friendly Tree-decomposition DP} 

First, we describe the desired contraction-friendly tree-decomposition DP for OCT. We are given an $n$-vertex graph $G=(V,E)$, a (possibly empty) subset $X\subseteq V$, and a tree-decomposition $\mathcal{T}$ of $G/X$. Let $T$ be the underlying tree of $\mathcal{T}$. For any $0\le l\le k$, we would like to decide whether there is a solution to OCT on $G$ of size $l$ which is disjoint from $X$. In particular, we would like to use the tree-decomposition $\mathcal{T}$ to solve this problem efficiently. For that purpose, first we define a subproblem on each vertex $t\in T$. As the bag $\beta(t)$ of $t$ might contain contracted vertices, we have to be careful in defining the subproblem. 

To define the subproblem, we need the following definition. For each subset $V'$ of vertices in $G/X$, let ${(G/X)(V')}^{-1}$ be the subgraph of $G$ that is the pre-image of ${(G/X)}[V']$, i.e., ${(G/X)(V')}^{-1}$ is obtained by undoing the contractions of all vertices in the induced subgraph ${(G/X)}[V']$. 
%Similarly, define ${(G/X)}^{-1}(\sigma(t))$. 

\begin{observation}\label{obs:distinct-config}
The number of distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ w.r.t. the solutions disjoint from $X$ is $2^{O(|V'|)}$. 
\end{observation} 

\begin{proof}
%Consider any solution $S$ of OCT disjoint from $X$ on any graph $G'$ that contains ${(G/X)}^{-1}(\sigma(t))$ as an induced subgraph. 
For each contracted vertex $v$ of $V'$, consider the connected component $C$ in $G[X]$ corresponding to $v$. Then as the solutions we seek are disjoint from $X$, $C$ must be bipartite. Hence, the number of distinct configuration of the vertices in $C$ w.r.t. such  solutions is only 2 depending on which partition is designated as the left or right. Also, any vertex $u$ of $V'\backslash X$ can have 3 configurations. Hence, the number of such distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ is at most $3^{|V'|}=2^{O(|V'|)}$.  
\end{proof}

Note that given ${(G/X)(V')}^{-1}$, one can easily compute the $2^{O(|V'|)}$ such configurations. For any solution $S$ and a configuration $\lambda$ of a set of vertices $V'$, we say $S$ is consistent with $\lambda$ if the 1-vertices of $V'$ are in $S$, and 2- and 3-vertices of $V'$ are in the left and right side of the residual bipartite graph. For any configuration $\lambda$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$ and $0\le l\le k$, we define a subproblem where the goal is to decide whether there is a solution to OCT on ${(G/X)(\gamma(t))}^{-1}$ which is disjoint from $X$, is consistent  with $\lambda$ and uses exactly $\ell$ vertices of ${(G/X)(\gamma(t)\backslash \sigma(t))}^{-1}$. Thus, in this subproblem, the solution contains 1-vertices of $\sigma(t)$ and $\ell$ additional vertices from ${(G/X)(\gamma(t)\backslash \sigma(t))}^{-1}$. We store the boolean value (YES/NO) of the solution of this subproblem in a table $L(t)$ indexed by $(\lambda,l)$. For simplicity, we assume wlog that all configurations are valid, i.e., for each configuration $\lambda$, 1-vertices of ${(G/X)(\sigma(t))}^{-1}$ come from $\mathsf{Cand}$. By Observation \ref{obs:distinct-config}, the number of entries that we need to store in $L(t)$ is $2^{O(|\sigma(t)|)}\cdot k$, and all such relevant configurations can be computed in $2^{O(|\sigma(t)|)}n^{O(1)}$ time. 

For our application, we cannot assume that the treewidth of $T$ is bounded. Instead, we make two assumptions: (i) the bag size of each non-leaf vertex in $T$ is bounded by a parameter $w$, and (ii) for each leaf $t\in T$, the table $L(t)$ is given to us. With these assumptions, we show that the table entries corresponding to all vertices of $T$ can be computed in time $2^{O(w)}n^{O(1)}$. 

Consider any non-leaf vertex $t\in T$. We can assume that the tables corresponding to the children of $t$ are already computed. Fix any configuration $\lambda$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$ and an integer $0\le l\le k$. We want to compute the entry in $L(t)$ w.r.t. $(\lambda,l)$. First, we guess a configuration $\lambda'$ of the vertices in ${(G/X)(\beta(t)\backslash \sigma(t))}^{-1}$ w.r.t. the solutions disjoint from $X$. Thus, we have the configuration of all vertices in $\beta(t)$. This gives us the configuration $\lambda(s)$ of $\sigma(s)$ for each child $s$ of $t$. We note that the vertices of $\beta(t)$ might be shared by multiple children. But, in our subproblems, the solution size does not account for the vertices in the adhesion. Thus, these solutions account for disjoint sets of vertices, and hence the subproblems can be treated as independent. Let $\ell^u$ be the number of 1-vertices in $\beta(t)\backslash \sigma(t)$ w.r.t. $\lambda'$. Then, we would like to compute a solution, which consists of these 1-vertices and $\ell_s$ vertices from ${(G/X)(\gamma(s)\backslash \sigma(s))}^{-1}$ for each child $s$ of $t$, where $\ell=\ell^u+\sum_s \ell_s$. Using the tables of the children, we can easily compute such a solution if possible, and hence the entry $(\lambda,l)$ can be computed in polynomial time. Now, as we need to enumerate all possible $2^{O(|\beta(t)\backslash \sigma(t)|)}$ configurations $\lambda'$, it is not hard to see that computation of each entry takes $2^{O(|\beta(t)\backslash \sigma(t)|)}n^{O(1)}$ time. Hence, the table for $t$ can be computed in time $2^{O(|\beta(t)|)}n^{O(1)}=2^{O(w)}n^{O(1)}$.  
     

% \begin{lemma}\label{lem:contraction-friendly}
% Suppose we are given a graph $G=(V,E)$, a (possibly empty) subset $X\subseteq V$, a subset $\mathsf{Cand}\subseteq V$, a tree-decomposition $\mathcal{T}$ of $G/X$ of width $w$, and an integer $\tau$, such that $G$ has a solution to OCT contained in $\mathsf{Cand}$ and of size $\tau$ that is disjoint from $X$. Then a solution to OCT on $G$ contained in $\mathsf{Cand}$, disjoint from $X$ and of size $\tau$ can be obtained in time $2^{O(w)}n^{O(1)}$.   
% \end{lemma}

\subsubsection{The Algorithm}
Now, we describe our main algorithm. First, we apply Lemma \ref{lem-rsdecomp} to compute in polynomial time a tree decomposition $\mathcal{T}_\textnormal{RS}$ of $G$ with adhesion size at most $h$ in which the torso of each vertex is $h$-almost-embeddable. Note that $h$ is a constant which depends only on $H$. Given $\mathcal{T}_\textnormal{RS}$, the idea is to employ a DP on it to solve OCT on $G$. However, we have to be careful here, as the width of $\mathcal{T}_\textnormal{RS}$ can be very large. Next, we describe our DP based algorithm to solve OCT on $\mathcal{T}_\textnormal{RS}$. 

Let ${T}_\textnormal{RS}$ be the underlying tree of $\mathcal{T}_\textnormal{RS}$. The DP algorithm stores a table $M(t)$ for each vertex $t \in {T}_\textnormal{RS}$. 
%We define a configuration $\lambda$ of $\sigma(t)$ to be a set of values corresponding to the vertices  in $\sigma(t)$, where each value is in $\{1,2,3\}$. We note that these three values denote whether the corresponding vertex $v$ is in the solution, is in the left side of the residual bipartite graph (after removing the solution OCT) or is in the right side of the residual bipartite graph. As we want our solution to be a subset of $\mathsf{Cand}$, the 1-vertices must always come from $\mathsf{Cand}$. Otherwise, we say the configuration is not valid. 
Each entry of $M(t)$ is indexed by a tuple $(\lambda,l)$ for a configuration $\lambda$ of $\sigma(t)$ and an integer $0\le l\le k$ which stores a boolean value YES/NO based on whether or not there is an OCT for $G[\gamma(t)]$ such that the OCT is consistent with $\lambda$ and uses exactly $\ell$ vertices of $\gamma(t)\backslash \sigma(t)$.
%, i.e., 1-vertices of $\sigma(t)$ are in the OCT, and 2- and 3-vertices of $\sigma(t)$ are in the left and right side of the residual bipartite graph. 
That is, the entry w.r.t. $(\lambda,l)$ stores the solution of the problem $\mathsf{Prob}_{\lambda,l}$ as defined in our framework. Note that the size of the table $M(t)$ is $O(k)$, as $\sigma(t)$ is at most the constant $h$. Next, we show how to compute the entries of $M(t)$. 

%In the base case, we compute the entries corresponding to the leaves of $\mathcal{T}_\textnormal{RS}$. Consider any such leaf $t$. Note that, by definition, $G[\beta(t)]$ itself is the torso of $t$, and hence is $h$-almost-embeddable. Fix any configuration $\lambda$ of $\sigma(t)$ and an integer $0\le l\le k$. We would like to compute the entry of $M(t)$ w.r.t. $(\lambda,l)$. The $l=0$ case is trivial. So, assume $l \ge 1$. If the entry w.r.t. $(\lambda,l-1)$ is YES, we can readily say the entry w.r.t. $(\lambda,l)$ is also YES. So, let us consider the other case. In this case, we apply Lemma~\ref{lem-key} on the graph $G[\beta(t)\backslash \gamma(t)]$ with $p = \lfloor \sqrt{k} \rfloor$ to obtain the disjoint sets $Z_1,\dots,Z_p$. Following the framework, for each $Z'$ that is a subset of some $Z_i\cap \mathsf{Cand}$, of size $O(k/p)=O(\sqrt{k})$, we solve OCT on the graph $G[\beta(t)]$ assuming the desired solution is disjoint from $Z_i\backslash Z'$. That is, we need to solve $\mathsf{Prob}_{\lambda,l,Z_i \backslash Z'}$. To do this, first we use the observation that $\mathbf{tw}(G[\beta(t)\backslash \gamma(t)]/(Z_i \backslash Z')) = O(p+|Z'|)=O(\sqrt{k})$, and compute a tree-decomposition $\mathcal{T}$ of $G[\beta(t)\backslash \gamma(t)]/(Z_i \backslash Z')$ of width $O(\sqrt{k})$. Note that we also want our solution to be consistent with the configuration $\lambda$. We know the 1-vertices $\sigma_1(t)\subseteq \sigma(t)$ are already selected in the solution. So, we just consider the subset $\sigma'(t)= \sigma(t)\backslash \sigma_1(t)$ and contract the connected components in $G[\sigma'(t)]$. Thereafter we add these contracted vertices to all bags of $\mathcal{T}$. Note that the treewidth of $\mathcal{T}$ still remains $O(\sqrt{k})$. Moreover, $\mathcal{T}$ is a tree-decomposition of $G[\beta(t)\backslash \sigma_1(t)]/X$ where $X=(Z_i \backslash Z')\cup \sigma'(t)$. Note that we need to compute an OCT of size at most $l$ in $G[\beta(t)\backslash \sigma_1(t)]$ such that the vertices in $(Z_i \backslash Z')\cup \sigma'(t)$ are disjoint from the desired solution. Hence, we apply Lemma \ref{lem:contraction-friendly} on $G[\beta(t)\backslash \sigma_1(t)]$ with $X$ and $\mathcal{T}$ as defined above, and $\tau=l$. If the algorithm in the lemma computes a valid solution, we set our entry $(\lambda,l)$ to YES and go to the next entry. Otherwise, we probe the next set $Z'$. Note that there can be $k^{O(\sqrt{k})}$ such set $Z'$ and the algorithm in Lemma \ref{lem:contraction-friendly} uses $2^{O(\sqrt{k})}n^{O(1)}$ time. Thus, computation of an entry $(\lambda,l)$ requires $k^{O(\sqrt{k})}n^{O(1)}$ time. It follows that the table of a leaf $t$ can be computed in the same time bound.       

%Let ${T}_\textnormal{RS}$ be the underlying tree of $\mathcal{T}_\textnormal{RS}$. 
Consider any vertex $t\in {T}_\textnormal{RS}$.   %Also fix a configuration $\lambda$ of $\sigma(t)$ and $1\le l\le k$. Again assume that the entry w.r.t. $(\lambda,l-1)$ stores NO. 
We can assume that the table entries corresponding to the children (if any) of $t$ are already computed. This is true, as in the base case, we deal with the leaves of ${T}_\textnormal{RS}$. First, we apply Corollary~\ref{cor-extention} on $t$ with $p = \lfloor \sqrt{k} \rfloor$ to obtain the sets $Y_1,\dots,Y_p \subseteq \gamma(t) \backslash \sigma(t)$. Then, following the framework, we construct the set $\varPi$ of pairs $(i,Y')$, where $i \in [p]$ and $Y' \subseteq Y_i$, satisfying three conditions: \textbf{(1)} $|\varPi| = |\mathsf{Cand}|^{O(\sqrt{k})}$, \textbf{(2)} $|Y'| = O(k/p)$ for all $(i,Y') \in \varPi$, and \textbf{(3)} for any configuration $\lambda$ of $\sigma(t)$ and $0\le l\le k$, the answer to $\mathsf{Prob}_{\lambda,l}$ is YES iff the answer to $\mathsf{Prob}_{\lambda,l,Y_i \backslash Y'}$ is YES for some $(i,Y') \in \varPi$. Thus, we can focus on a fixed set $Y'\subseteq Y_i$ and solve $\mathsf{Prob}_{\lambda,l,Y_i \backslash Y'}$ for all $\lambda$ and $l$. Again, following the framework, we apply Lemma \ref{lem-specialtd} to obtain a tree-decomposition $\mathcal{T}^*$ of $G[\gamma(t)]/(Y_i \backslash Y')$ in time $2^{O(\sqrt{k})} n^{O(1)}$. Any non-leaf vertex in the underlying tree ${T}^*$ of $\mathcal{T}^*$ has bag size $O(\sqrt{k})$. However, for a leaf, the bag size can be large. Nevertheless, by Property \textbf{(iii)} in Lemma \ref{lem-specialtd}, for such a leaf $t^* \in {T}^*$, $\gamma(t^*) = \beta(t^*) = \gamma(s)$ and $\sigma(t^*) = \sigma(s)$ for some $s \in C_i$. Recall that $C_i$ is the set of children $s$ of $t$ satisfying $\gamma(s) \cap Y_i = \emptyset$. Thus, by our assumption, the table $M(t^*)$ corresponding to $t^*$ is already computed. Subsequently, we apply the contraction-friendly DP on the tree-decomposition $\mathcal{T}^*$. 
%, and $\tau=l$. Note that Lemma \ref{lem:contraction-friendly} demands a tree-decomposition of bounded width, which $\mathcal{T}^*$ does not have. However, using the observation above regarding leaves of $T^*$, one can trivially adapt the proof of Lemma \ref{lem:contraction-friendly} to handle this special case. 
Now, by Property \textbf{(ii)} in Lemma \ref{lem-specialtd}, the root $\mathsf{rt}$ of $T^*$ has only one child $\mathsf{rt}'$, where $\sigma(\mathsf{rt}') = \sigma(t)$ and $ \beta(\mathsf{rt}) = \sigma(t)$. Also, note that $\sigma(t)\cap Y_i=\emptyset$, and so $\sigma(t)\cap (Y_i \backslash Y')=\emptyset$. Thus, the vertices of $\sigma(t)$ are not contracted in  $\mathcal{T}^*$. Hence, 
%$\beta(\mathsf{rt}) = \sigma(t)$, where  $\mathsf{rt}$ is the root of $T^*$. 
the table $L(\mathsf{rt}')$ computed by the contraction-friendly DP contains entries corresponding to all possible configurations of $\sigma(\mathsf{rt}') = \sigma(t)$ and all $0\le l\le k$. Thus, this is exactly the table needed for $t$, and  we can just set $M(t)[\lambda,l]\leftarrow M(t)[\lambda,l] \lor L(\mathsf{rt}')[\lambda,l]$ for each configuration $\lambda$ of $\sigma(t)$ and $0\le l\le k$. Note that in our solutions, we do not count the vertices of $\sigma(t)$. But, this can be easily fixed at the end by adding the  1-vertices for each configuration to the computed solution and computing the best combined solution.   

Now, the contraction-friendly DP takes $2^{O(w)}n^{O(1)}$ time, where $w$ is the bag size of any non-leaf vertex in $T^*$. Also, the total number of pairs $(i,Y')$ in $\varPi$ is ${|\textsf{Cand}|}^{O(\sqrt{k})}n^{O(1)}$. Thus, the computation of $M(t)$ takes in total $|\textsf{Cand}|^{O(\sqrt{k})}\cdot 2^{O(w)}\cdot n^{O(1)}$ time. As the bag size of any non-leaf vertex in ${T}^*$ is $O(\sqrt{k})$, a trivial upper bound on this is $n^{O(\sqrt{k})}$. Also, by Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for OCT is $k^{O(1)}$. Subsequently, we obtain the time bound of $2^{O(\sqrt{k}\log k)}n^{O(1)}$. It follows that the OCT problem on $G$ can be solved in the same time bound. 

\begin{theorem}
\probOCT on $H$-minor free graphs can be solved in $2^{O(\sqrt{k}\log k)}n^{O(1)}$ time. 
\end{theorem}

\subsubsection{\probEB}
The \probEB (EB) problem is similar to OCT, except here we need to remove a subset of edges. Formally, we are given an $H$-minor-free graph $G=(V,E)$ and a parameter $k$, and we would like to decide whether there is a subset $E'\subseteq E$ of size at most $k$ such that removal of the edges in $E'$ from $G$ gives us a bipartite graph. As we saw in the previous subsection, the main ingredient for applying the framework is the contraction-friendly tree-decomposition DP. Here, we describe such a DP for EB. The rest of the algorithm is similar to the one for OCT. 

% If there is such a subset, we refer to it as a solution. By abusing the notation, we refer to a solution to the OCT problem also as an OCT. The distinction should be clear from the context. Following our framework, the first step is to apply Lemma~\ref{lem-candidate} to obtain a candidate set $\mathsf{Cand} \subseteq V$ of size $k^{O(1)}$ for the instance. Note that this takes only a polynomial time. For our purpose, it is sufficient to find a solution which is a subset of $\mathsf{Cand}$. Henceforth, by the term solution we always mean a subset of $\mathsf{Cand}$.       

Consider any subgraph $G_1=(V_1,E_1)$ and fix any solution $E_\mathsf{sol}$ on $G_1$. We say that $E_\mathsf{sol}$ is disjoint from a set of vertices $X$ if the endpoints of the edges in $E_\mathsf{sol}$ are disjoint from $X$. We define a configuration $\lambda$ of $V'\subseteq V_1$ w.r.t. the solution to be a set of values corresponding to the vertices  in $V'$, where each value is in $\{1,2\}$. We note that these values denote whether the corresponding vertex $v$ is in the left side of the residual bipartite graph (after removing the solution edges) or is in the right side of the residual bipartite graph. Next, we describe the contraction-friendly tree-decomposition DP for EB.  

We are given an $n$-vertex graph $G=(V,E)$, a (possibly empty) subset $X\subseteq V$, and a tree-decomposition $\mathcal{T}$ of $G/X$. Let $T$ be the underlying tree of $\mathcal{T}$. For any $0\le l\le k$, we would like to decide whether there is a solution to EB on $G$ of size $l$ which is disjoint from $X$. The following observation is similar to Observation \ref{obs:distinct-config}. 

\begin{observation}\label{obs:distinct-config-EB}
The number of distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ w.r.t. the solutions disjoint from $X$ is $2^{O(|V'|)}$. 
\end{observation} 

For any solution $S$ and a configuration $\lambda$ of a set of vertices $V'$, we say $S$ is consistent with $\lambda$ if the 1- and 2-vertices of $V'$ are in the left and right side of the residual bipartite graph. For any configuration $\lambda$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$ and $0\le l\le k$, we define a subproblem where the goal is to decide whether there is a solution to EB on ${(G/X)(\gamma(t))}^{-1}$ which is disjoint from $X$, consistent with $\lambda$ and uses exactly $\ell$ edges such that at least one endpoint of each edge is not in ${(G/X)(\sigma(t))}^{-1}$. Thus, in this subproblem, the solution contains the edges whose both endpoints are 1-vertices (or 2-vertices) among the set of edges $E^1$ in ${(G/X)(\sigma(t))}^{-1}$ and $\ell$ additional edges from ${(G/X)(\gamma(t))}^{-1}$ which are not in $E^1$. We store the boolean value (YES/NO) of the solution of this subproblem in a table $L(t)$ indexed by $(\lambda,l)$. 

We note that it is sufficient to solve the above subproblem, as the edges used in a solution from ${(G/X)(\sigma(t))}^{-1}$ can be easily derived from the corresponding configuration. The subproblem is defined in this way to avoid any potential multiple counting of a solution edge at different levels. In this setting, if an edge $(u,v)$ is common to both parent and child subproblems, the decision to take it or not is uniquely determined by the configuration corresponding to the children. 

By Observation \ref{obs:distinct-config-EB}, the number of entries that we need to store in $L(t)$ is $2^{O(|\sigma(t)|)}\cdot k$, and all such relevant configurations can be computed in $2^{O(|\sigma(t)|)}n^{O(1)}$ time. With these modified definitions of subproblem and DP table, the rest of the algorithm is similar to  the one for OCT. Hence, we conclude that the table entries corresponding to all vertices of $T$ can be computed in time $2^{O(w)}n^{O(1)}$, where $w$ is the maximum size of the bags of the non-leaf vertices in $T$. 

Note that by our framework, the total running time of our algorithm is $(|\textsf{Cand}|^{O(\sqrt{k})}\cdot 2^{O(w)})\cdot n^{O(1)}$, where $w=\sqrt{k}$. By Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for EB is $k^{O(1)}$. Subsequently, we obtain the time bound of $2^{O(\sqrt{k}\log k)}n^{O(1)}$.  

\begin{theorem}
\probEB on $H$-minor free graphs can be solved in $2^{O(\sqrt{k}\log k)}n^{O(1)}$ time. 
\end{theorem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{\probGFVS and \probGFES}
For a directed graph $G=(V,A)$, a finite group $\Sigma$ of size $g$ and a labeling function $\Lambda: A\rightarrow \Sigma$, $(G,\Lambda)$ is called a $\Sigma$-labeled graph if for each arc $(u,v)\in A$, $(v,u)$ is also in $A$ and $\Lambda((u,v))=\Lambda((v,u))^{-1}$. For a subset of vertices $D$, we denote by $(G\backslash D,\Lambda)$ the $\Sigma$-graph obtained by removing the vertices in $D$ from $(G,\Lambda)$. Similarly, for a subset of arcs $A'$, we denote by $(G\backslash A',\Lambda)$ the $\Sigma$-labeled graph obtained by removing the arcs in $A'$ from $(G,\Lambda)$. For a cycle $C=\{v_1,\ldots,v_t,v_1\}$, let $\Lambda(C)=\Lambda((v_1,v_2))\cdot \ldots \cdot \Lambda((v_{t-1},v_t))\cdot \Lambda((v_t,v_1))$. Here $\cdot $ is the group operation. A cycle $C$ is called a non-null cycle if $\Lambda(C)\ne 1_{\Sigma}$. In the \probGFVS (GFVS) problem, given a $\Sigma$-labeled graph $(G,\Lambda)$ and a parameter $k$, the goal is to decide whether there is a set of vertices $D$ such that $(G\backslash D,\Lambda)$ does not have any non-null cycle. The \probGFES (GFES) problem is similar, except here the goal is to decide whether there is a set of arcs $A'$ such that $(G\backslash A',\Lambda)$ does not have any non-null cycle. For simplicity, we assume that $\Sigma=\{1,\ldots,g\}$.  

First, we apply our framework on GFVS. We note that OCT is a specialization of GFVS when $\Sigma=\{0,1\}$ \cite{KratschW20}. Indeed, our algorithm for GFVS is an extension of the algorithm for OCT. In the following, we just describe the contraction-friendly tree-decomposition DP for GFVS. The remaining algorithm is similar to the one for OCT. Following our framework, the first step is to obtain a candidate set $\mathsf{Cand} \subseteq V$. Henceforth, by the term solution we always mean a subset of $\mathsf{Cand}$.       

For describing our algorithm, we need a definition. For a $\Sigma$-labeled graph $(G,\Lambda)$, $\mu: V\rightarrow \Sigma$ is called a consistent labeling iff for each arc $(u,v)$ in $G$, we have $\mu(v)=\mu(u)\cdot \Lambda((u,v))$. 

\begin{lemma}\label{lem:consistentlabels}
\cite{Guillemot11a} A $\Sigma$-labeled graph has a consistent labeling iff it does not contain any non-null cycle. 
\end{lemma}

Consider any subgraph $G_1=(V_1,A_1)$ and fix any solution $S$ of GFVS on $G_1$. Also, consider a consistent labeling $\mu$ of the vertices in the graph $(G\backslash D,\Lambda)$, which exists by the above lemma. We define a configuration $\lambda$ of $V'\subseteq V_1$ w.r.t. $S$ to be a set of values corresponding to the vertices in $V'$, where each value is in $\{0,1,\ldots,g\}$. We note that these values denote whether the corresponding vertex $v$ is in the solution (0) or is mapped to the element $i\in \Sigma$ via $\mu$. As we want our solution to be a subset of $\mathsf{Cand}$, the 0-vertices must always come from $\mathsf{Cand}$. We also say that $S$ is \emph{compatible} with the configuration $\lambda$.  


\begin{observation}\label{obs:distinct-config-gfvs}
The number of distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ w.r.t. the solutions disjoint from $X$ is $g^{O(|V'|)}$. 
\end{observation} 

\begin{proof}
%Consider any solution $S$ of OCT disjoint from $X$ on any graph $G'$ that contains ${(G/X)}^{-1}(\sigma(t))$ as an induced subgraph. 
For each contracted vertex $v$ of $V'$, consider the connected component $C$ in $G[X]$ corresponding to $v$. Then as the solutions we seek are disjoint from $X$, $C$ must have no non-null cycles. It follows that the vertices of $C$ has a consistent labeling $\mu$. Now, fix the label of any vertex in $C$. By definition of consistent labeling, this also fixes the labeling of the remaining vertices of $C$. Thus, the number of distinct labelings of the vertices of $C$ is only $g$. Hence, the number of distinct configurations of the vertices in $C$ w.r.t. the solutions disjoint from $X$ is only $g$. Also, any vertex $u$ of $V'\backslash X$ can have $g+1$ configurations. Hence, the number of such distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ is at most $(g+1)^{|V'|}=g^{O(|V'|)}$.  
\end{proof}

Next, we describe the contraction-friendly tree-decomposition DP for GFVS. A subproblem is defined in the same way as for OCT. For any configuration $\lambda$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$ and $0\le l\le k$, we define a subproblem where the goal is to decide whether there is a solution to GFVS on ${(G/X)(\gamma(t))}^{-1}$ which is disjoint from $X$, is compatible with $\lambda$ and  uses exactly $\ell$ vertices of ${(G/X)(\gamma(t)\backslash \sigma(t))}^{-1}$. We store the boolean value (YES/NO) of the solution of this subproblem in a table $L(t)$ indexed by $(\lambda,l)$. For simplicity, we assume wlog that all configurations are valid, i.e., for each configuration $\lambda$, 1-vertices of ${(G/X)(\sigma(t))}^{-1}$ come from $\mathsf{Cand}$. 
By Observation \ref{obs:distinct-config-gfvs}, the number of entries that we need to store in $L(t)$ is $g^{O(|\sigma(t)|)}\cdot k$, and all such relevant configurations can be computed in $g^{O(|\sigma(t)|)}n^{O(1)}$ time. With these modified definitions of subproblem and DP table, the rest of the algorithm is similar to  the one for OCT. Hence, we conclude that the table entries corresponding to all vertices of $T$ can be computed in time $g^{O(w)}n^{O(1)}$, where $w$ is the maximum size of the bags of the non-leaf vertices in $T$. 

Note that by our framework, the total running time of our algorithm is $(|\textsf{Cand}|^{O(\sqrt{k})}\cdot g^{O(w)})\cdot n^{O(1)}$, where $w=\sqrt{k}$. A trivial upper bound on this is $(ng)^{O(\sqrt{k})}$. Also, by Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for GFVS is $k^{O(g)}$. Subsequently, we obtain the time bound of $2^{O(g \sqrt{k}\log(gk))} \cdot n^{O(1)}$.  

\begin{theorem}
\probGFVS on $H$-minor free graphs can be solved in $\min\{(ng)^{O(\sqrt{k})},$ $2^{O(g \sqrt{k}\log(gk))} \cdot n^{O(1)}\}$ time. 
\end{theorem}


\subsubsection{\probGFES}
The algorithm for GFES is similar to the one for GFVS. Here, we describe the main differences. For simplicity, we use the terms edge and arc interchangeably. Consider any subgraph $G_1=(V_1,E_1)$ and fix any solution $E_\mathsf{sol}$ on $G_1$. We say that $E_\mathsf{sol}$ is disjoint from a set of vertices $X$ if the endpoints of the edges in $E_\mathsf{sol}$ are disjoint from $X$. Consider a consistent labeling $\mu$ of the vertices in the graph $(G\backslash E_\mathsf{sol},\Lambda)$, which exists by Lemma \ref{lem:consistentlabels}. We define a configuration $\lambda$ of $V'\subseteq V_1$ w.r.t. $E_\mathsf{sol}$ to be a set of values corresponding to the vertices in $V'$, where each value is in $\{1,\ldots,g\}$. We note that these values denote whether the corresponding vertex $v$ is mapped to the element $i\in \Sigma$ via $\mu$. We also say that $S$ is \emph{compatible} with the configuration $\lambda$. The following observation is similar to Observation \ref{obs:distinct-config-gfvs}.  


\begin{observation}\label{obs:distinct-config-gfes}
The number of distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ w.r.t. the solutions disjoint from $X$ is $g^{O(|V'|)}$. 
\end{observation} 

Next, we describe the contraction-friendly tree-decomposition DP for GFES. For any configuration $\lambda$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$ and $0\le l\le k$, we define a subproblem where the goal is to decide whether there is a solution to GFES on ${(G/X)(\gamma(t))}^{-1}$ which is disjoint from $X$, consistent with $\lambda$ and uses exactly $\ell$ edges such that at least one endpoint of each edge is not in ${(G/X)(\sigma(t))}^{-1}$. We store the boolean value (YES/NO) of the solution of this subproblem in a table $L(t)$ indexed by $(\lambda,l)$. By Observation \ref{obs:distinct-config-gfes}, the number of entries that we need to store in $L(t)$ is $g^{O(|\sigma(t)|)}\cdot k$, and all such relevant configurations can be computed in $g^{O(|\sigma(t)|)}n^{O(1)}$ time. With these modified definitions of subproblem and DP table, the rest of the algorithm is similar to  the one for EB. Hence, we conclude that the table entries corresponding to all vertices of $T$ can be computed in time $g^{O(w)}n^{O(1)}$, where $w$ is the maximum size of the bags of the non-leaf vertices in $T$. 

Note that by our framework, the total running time of our algorithm is $(|\textsf{Cand}|^{O(\sqrt{k})}\cdot g^{O(w)})\cdot n^{O(1)}$, where $w=\sqrt{k}$. A trivial upper bound on this is $(ng)^{O(\sqrt{k})}$. Also, by Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for GFES is $k^{O(\log^3 k)}$. Subsequently, we obtain the time bound of $2^{O(\sqrt{k} \log g \log^4 k)} \cdot n^{O(1)}$.  

\begin{theorem}
\probGFES on $H$-minor free graphs can be solved in $\min\{(ng)^{O(\sqrt{k})},$ $2^{O(\sqrt{k} \log g \log^4 k)} \cdot n^{O(1)}\}$ time. 
\end{theorem}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    

\subsection{\probVMultiC and \probEMultiC}
In \probVMultiC (VMC), given a graph $G=(V,E)$, a collection $U$ of $r$ pairs of vertices $U \subseteq V \times V$, and an integer $k$, the goal is to decide if there is a set of $k$ vertices of $V \backslash R$ whose removal separates each pair of vertices in $U$ where $R$ is the set of vertices appearing in the pairs of $U$. \probEMultiC (EMC) is similar, except here we remove a set of $k$ edges. Here $R$ is called the set of terminals. First, we consider VMC. Following our framework, the first step is to obtain a candidate set $\mathsf{Cand} \subseteq V$. Henceforth, by the term solution we always mean a subset of $\mathsf{Cand}$. Next, we describe the contraction-friendly tree-decomposition DP for VMC. Our DP is a natural extension of a DP for bounded treewidth graphs \cite{GuoHKNU08}. 

We are given an $n$-vertex graph $G=(V,E)$, a (possibly empty) subset $X\subseteq V$, and a tree-decomposition $\mathcal{T}$ of $G/X$. Let $T$ be the underlying tree of $\mathcal{T}$. We would like to solve a subproblem in ${(G/X)(\gamma(t))}^{-1}$. Consider any partition $\Pi$ of $R$ such that each pair in $U$ appears in two different parts. We can have $|R|^{O(|R|)}=r^{O(r)}$ such distinct partitions. Note that each such partition helps us guess which terminals will be on the same connected component after removal of a solution. We  define subproblems with respect to $\Pi$, assuming $\Pi$ is the correct configuration of the terminals. Let $\alpha\le 2r$ be the number of parts. We treat each part as a color between $1$ to $\alpha$. 

Consider any subgraph $G_1=(V_1,E_1)$ and fix any solution $S$ on $G_1$. We define a configuration $\lambda$ of $V'\subseteq V_1$ w.r.t. the solution to be a set of values corresponding to the vertices in $V'$, where each value is in $\{0,1,2,\ldots,\alpha\}$. We note that these values denote whether the corresponding vertex $v$ is in $S$ (0), or is in the $i$-th connected component along with the vertices of $R$ in $i$-th part ($i$). We say that $S$ is consistent with $\lambda$.  

\begin{observation}\label{obs:distinct-config-vmc}
The number of distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ w.r.t. the solutions disjoint from $X$ is ${\alpha}^{O(|V'|)}$. 
\end{observation} 

\begin{proof}
%Consider any solution $S$ of OCT disjoint from $X$ on any graph $G'$ that contains ${(G/X)}^{-1}(\sigma(t))$ as an induced subgraph. 
For each contracted vertex $v$ of $V'$, consider the connected component $C$ in $G[X]$ corresponding to $v$. Then as the solutions we seek are disjoint from $X$, all vertices in $X$ have the same value in any configuration w.r.t. such a solution. Hence, the number of distinct configurations of the vertices in $C$ w.r.t. such  solutions is only $\alpha$ depending on the connected component in which they end up. Also, any vertex $u$ of $V'\backslash X$ can have at most $\alpha+1$ configurations. Hence, the number of such distinct configurations of the vertices in ${(G/X)(V')}^{-1}$ is at most ${(\alpha+1)}^{|V'|}={\alpha}^{O(|V'|)}$.  
\end{proof}

For any configuration $\lambda$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$ and $0\le l\le k$, we define a subproblem where the goal is to decide whether there is a solution to VMC on ${(G/X)(\gamma(t))}^{-1}$ which is disjoint from $X$, is consistent  with $\lambda$ and uses exactly $\ell$ vertices of ${(G/X)(\gamma(t)\backslash \sigma(t))}^{-1}$. We store the boolean value (YES/NO) of the solution of this subproblem in a table $L(t)$ indexed by $(\lambda,l)$. By Observation \ref{obs:distinct-config-vmc}, the number of entries that we need to store in $L(t)$ is $r^{O(|\sigma(t)|)}\cdot k$, and all such relevant configurations can be computed in $r^{O(|\sigma(t)|)}n^{O(1)}$ time. With these modified definitions of subproblem and DP table, the rest of the algorithm is similar to  the one in \cite{GuoHKNU08}. Hence, we conclude that the table entries corresponding to all vertices of $T$ can be computed in time $r^{O(r+w)}n^{O(1)}$, where $w$ is the maximum size of the bags of the non-leaf vertices in $T$. 

Note that by our framework, the total running time of our algorithm is $(|\textsf{Cand}|^{O(\sqrt{k})}\cdot r^{O(r+w)})\cdot n^{O(1)}$, where $w=\sqrt{k}$. A trivial upper bound on this is $n^{O(\sqrt{k}+r)}$, as $r\le n^2$. Also, by Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for VMC is $k^{O(\sqrt{r})}$. Subsequently, we obtain the time bound of $2^{O(r\sqrt{k} \log k)} \cdot n^{O(1)}$.  

\begin{theorem}
\probVMultiC on $H$-minor free graphs can be solved in 
$\min\{n^{O(\sqrt{k}+r)}, 
2^{O((\sqrt{rk}+r) \log rk))} \cdot n^{O(1)}
\}$ 
time. 
\end{theorem}


As mentioned in \cite{GuoHKNU08}, the DP for VMC is almost the same as the DP for EMC. Similarly, the contraction-friendly tree-decomposition DP for EMC is very similar to the one for VMC. Also, the candidate set size for EMC is $(r+k)^{O(\log^3(r+k))}$. Hence, we obtain the following theorem. 

\begin{theorem}
\probEMultiC on $H$-minor free graphs can be solved in 
$\min\{n^{O(\sqrt{k}+r)}, 
2^{O((r+\sqrt{k})\log^4 (rk))} \cdot n^{O(1)}
\}$ 
time.
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{\probVMC and \probEMC}
In \probVMC (VMWC), given a graph $G$, a subset of $r$ vertices $R \subseteq V (G)$, called terminals, and an integer $k$, the goal is to decide if there is a set of at most $k$ vertices of $V(G) \backslash R$ hitting every path between a pair of terminals. \probEMC (EMWC) is similar, except the goal is to decide if there is a set of at most $k$ edges of $E(G)$ hitting every path between a pair of terminals. 

Note that VMWC is a special case of VMC where we have to separate all $r^2$ pairs of terminals in $R\times R$. Also, we need to consider only one partition where each terminal belongs to a separate part. Thus, we readily obtain a contraction free DP that runs in $r^{O(w)}n^{O(1)}$ time.  

By our framework, the total running time of our algorithm is $(|\textsf{Cand}|^{O(\sqrt{k})}\cdot r^{O(w)})\cdot n^{O(1)}$, where $w=\sqrt{k}$. A trivial upper bound on this is $n^{O(\sqrt{k})}$, as $r\le n$. Also, by Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for VMWC is $k^{O(r)}$. Subsequently, we obtain the time bound of $2^{O(r\sqrt{k} \log k)} \cdot n^{O(1)}$.  

\begin{theorem}
\probVMC on $H$-minor free graphs can be solved in $\min\{n^{O(\sqrt{k})},$ $2^{O(r\sqrt{k} \log k)} \cdot n^{O(1)}\}$ time. 
\end{theorem}

\subsection{\probEMC}
We describe the contraction-friendly tree-decomposition DP for EMWC. This DP is partly motivated by the DP in \cite{DengLZ13} for Multi-Multiway cut which is a generalization of EMWC. We are given an $n$-vertex graph $G=(V,E)$, a (possibly empty) subset $X\subseteq V$, and a tree-decomposition $\mathcal{T}$ of $G/X$. Let $T$ be the underlying tree of $\mathcal{T}$. Consider any non-leaf vertex $t \in T$. Note that removal of the solution edges in EMWC induces a partition of the vertices where each part (or connected component) contains at most one terminal of $R$. We would like to guess an optimal partition. Consider any subset $V' \subseteq \beta(t)$, and any partition $\Pi=\{X_i\mid i\in I\}$ of the vertices in ${(G/X)(V')}^{-1}$ for some index set $I$. We say a set of edges $C$ in ${(G/X)(\gamma(t))}^{-1}$ is consistent with $\Pi$ and vice versa iff 
\begin{itemize}
    \item The endpoints of the edges in $C$ are disjoint from $X$;
    \item $C$ separates all the terminals; and
    \item Let $G'$ be the subgraph ${(G/X)(\gamma(t))}^{-1}$ after removing the edges in $C$. Let $\{P_i\mid i\in I\}$ be the family of connected components such that $P_i\cap V'\ne \emptyset$ for all $i\in I$. Then $X_i=P_i$ for all $i\in I$. 
\end{itemize}

\begin{observation}\label{obs:distinct-config-emwc}
The number of distinct partitions of the vertices in ${(G/X)(V')}^{-1}$ consistent with sets of edges is ${|V'|}^{O(|V'|)}$.
\end{observation} 

\begin{proof}
%Consider any solution $S$ of OCT disjoint from $X$ on any graph $G'$ that contains ${(G/X)}^{-1}(\sigma(t))$ as an induced subgraph. 
First note that the number of distinct partitions of the vertices in $V'$ is ${|V'|}^{O(|V'|)}$. However, $(G/X)$ $(V'){}^{-1}$ might contain many more vertices, as we undo the contraction of the component vertices in $V'$. For each contracted vertex $v$ of $V'$, consider the connected component $C$ in $G[X]$ corresponding to $v$. Then as the endpoints of the edges in consistent sets $C$ are disjoint from $X$, all vertices in $X$ must end up in the same connected component after removal of the edges from $C$. It follows that the number of such distinct partitions of the vertices in ${(G/X)(V')}^{-1}$ is again bounded by ${|V'|}^{O(|V'|)}$. 
\end{proof}

For any partition $\Pi$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$, we define a subproblem where the goal is to find the minimum size set of edges $C$ in ${(G/X)(\gamma(t))}^{-1}$ which is consistent with $\Pi$. It is sufficient to solve this subproblem for our purpose, as if we know the minimum value, we can also solve the decision version of the problem. We store a solution $C$ of this subproblem in a table $L(t)$ indexed by $\Pi$. To compute the table corresponding to $t$, we need to merge the tables of its children. In the following, we describe how to merge the tables of two children. One can easily extend it to more than two children.  

Consider any partition $\Pi_1$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$. We extend this partition to obtain a partition $\Pi_2$ of the vertices in ${(G/X)(\beta(t))}^{-1}$. For the purpose of extension, we define compatibility of two partitions. Consider two partitions  $\Pi_1=\{X_i\mid i\in I\}$ and $\Pi_2=\{Y_j\mid j\in J\}$. Also, consider the bipartite graph $B=(I,J,E')$ such that $(i,j)\in E'$ iff $X_i\cap Y_j\ne \emptyset$. Then $\Pi_1$ and $\Pi_2$ are compatible if $E'$ is a perfect matching and for each edge $(i,j)\in E'$, $i=j$. 
%Consider such a mergeable pair. For $(i,i)\in E'$, let $Z_i=(X_i\cup Y_i)\cap \beta(t)$. Let $\Pi=\cup_i Z_i$. We denote $\Pi$ by $\Pi_1\xor \Pi_2$. 

Now, fix a partition $\Pi$ of the vertices in ${(G/X)(\sigma(t))}^{-1}$. We show how to compute the entry $L(t)[\Pi]$ by merging tables of two children $s_1$ and $s_2$. First, we take a partition $\Pi'$ of the vertices in ${(G/X)(\beta(t))}^{-1}$ which is compatible with $\Pi$. Given $\Pi'$, the partition of the vertices in  ${(G/X)(\sigma(s_1))}^{-1}$ (or ${(G/X)(\sigma(s_2))}^{-1}$) compatible with $\Pi'$, is also fixed. Let $\Pi_1$ and $\Pi_2$ be these two partitions w.r.t. $s_1$ and $s_2$. The entry $L(t)[\Pi]=\arg \min_{|C|} \{C=L(s_1)[\Pi_1]\cup L(s_2)[\Pi_2]\cup C'\}$, where $C'$ is a subset of edges $\{(u,v)\mid u,v \notin X\}$ such that $(u,v)$ is in ${(G/X)(\beta(t))}^{-1}$, but not in ${(G/X)(\gamma(s_1))}^{-1}$ or ${(G/X)(\gamma(s_2))}^{-1}$, and $u$ and $v$ are contained in different parts of $\Pi'$.   

The correctness follows from the fact that if an edge $(u,v)$ is common to both parent and child subproblems, the decision to take it or not is uniquely determined by the partition corresponding to the children. Thus, no edge is counted more than once in the computed solution.  

Note that computation of a table entry requires enumerating all possible $\Pi'$. The number of such partitions is bounded by $w^{O(w)}$ by Observation \ref{obs:distinct-config-emwc}, where $w$ is the maximum size of the bags of the non-leaf vertices in $T$. By the same observation, the number of entries that we need to store in $L(t)$ is ${|\sigma(t)|}^{O(|\sigma(t)|)}\cdot k$, and all such relevant partitions can be computed in ${|\sigma(t)|}^{O(|\sigma(t)|)}n^{O(1)}$ time. Hence, we conclude that the table entries corresponding to all vertices of $T$ can be computed in time $w^{O(w)} n^{O(1)}$. 

By our framework, the total running time of our algorithm is $(|\textsf{Cand}|^{O(\sqrt{k})}\cdot w^{O(w)})\cdot n^{O(1)}$, where $w=\sqrt{k}$. A trivial upper bound on this is $n^{O(\sqrt{k})}$. Also, by Lemma \ref{lem-candidate}, the size of $\textsf{Cand}$ for EMWC is $k^{O(\log^3 k)}$. Subsequently, we obtain the time bound of $2^{O(\sqrt{k}\log^4 k)} \cdot n^{O(1)}$.  

\begin{theorem}
\probEMC on $H$-minor free graphs can be solved in $2^{O(\sqrt{k}\log^4 k)} \cdot n^{O(1)}$ time. 
\end{theorem}


==> Saket/saketPreamble.tex <==
%\usepackage{microtype}%if unwanted, comment out or use option "draft"
\usepackage{wrapfig}
\usepackage{bm}

\usepackage{graphicx,color}
\usepackage{empheq}
\usepackage{tcolorbox}
\definecolor{blueish}{rgb}{0.122, 0.435, 0.698}
\definecolor{dagstuhlyellow}{rgb}{0.99,0.78,0.07}
\definecolor{lightgray}{rgb}{0.9,0.9,0.9}
\newtcbox{\colbox}{
size=title,
  nobeforeafter,
  colframe=white,
  colback=blue!5!white,
  arc=10pt,
  tcbox raise base}
  
  
  
\newcommand{\defparproblemR}[4]{
  \vspace{1mm}
\noindent\colbox{
  \begin{minipage}{0.94\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  &
    {\textbf{Parameter:}} #3 \\ \end{tabular*}
  {\textbf{Input:}} #2  \\
  {\textbf{Task:}} #4
  \end{minipage}
  }
 % \vspace{1mm}
}

%\newcommand{\defparproblemRNP}[4]{
% % \vspace{1mm}
%  \begin{center}
%\noindent\colbox{
%  \begin{minipage}{0.44\textwidth}
%  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  \end{tabular*}
%  {\textbf{Input:}} #2  \\
%  {\textbf{Task:}} #3
%  \end{minipage}
%  }
%\end{center}
% % \vspace{1mm}
%}




\newcommand{\defparproblemRNP}[3]{
  \begin{center}
\noindent\colbox{
  \begin{minipage}{0.85\textwidth}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  \end{tabular*}
  {\textbf{Input:}} #2  \\
  {\textbf{Task:}} #3
  \end{minipage}
  }
\end{center}
}


\usepackage{xspace}
\newcommand{\pname}{\textsc}
\newcommand{\ProblemFormat}[1]{\pname{#1}}
\newcommand{\ProblemIndex}[1]{\index{problem!\ProblemFormat{#1}}}
\newcommand{\ProblemName}[1]{\ProblemFormat{#1}\ProblemIndex{#1}{}\xspace}

\newcommand{\probPVD}{\ProblemName{Planar Vertex Deletion}}
\newcommand{\probCVD}{\ProblemName{Chordal Vertex Deletion}}
\newcommand{\probEB}{\ProblemName{Edge Bipartization}}
\newcommand{\probOCT}{\ProblemName{Odd Cycle Transversal}}
\newcommand{\probEMC}{\ProblemName{Edge Multiway Cut}}
\newcommand{\probVMC}{\ProblemName{Vertex Multiway Cut}}
\newcommand{\probVrMC}{\ProblemName{Vertex $r$-Multiway Cut}}
\newcommand{\probGFVS}{\ProblemName{Group Feedback Vertex Set}}
\newcommand{\probGFES}{\ProblemName{Group Feedback Edge Set}}
\newcommand{\probGFEVS}{\ProblemName{Group Feedback Edge/Vertex Set}}
\newcommand{\probEMultiC}{\ProblemName{Edge Multicut}}
\newcommand{\probErMultiC}{\ProblemName{Edge $r$-Multicut}}
\newcommand{\probVMultiC}{\ProblemName{Vertex Multicut}}
\newcommand{\probVrMultiC}{\ProblemName{Vertex $r$-Multicut}}
\newcommand{\probEVMultiC}{\ProblemName{Edge/Vertex Multicut}}
\newcommand{\probSFVS}{\ProblemName{Subset Feedback Vertex Set}}

\newcommand{\probTWdel}{\ProblemName{Treewidth-$\eta$ Modulator}}
\newcommand{\probFdel}{\ProblemName{$\mathcal{F}$-Deletion}}
\newcommand{\probFpack}{\ProblemName{$\mathcal{F}$-Packing}}
\newcommand{\probSdel}{\ProblemName{$\mathcal{S}$-Deletion}}
\newcommand{\probSpack}{\ProblemName{$\mathcal{S}$-Packing}}
% Commonly used names
\newcommand{\probVC}{\ProblemName{Vertex Cover}}
\newcommand{\probPlVC}{\ProblemName{Planar Vertex Cover}}
\newcommand{\probPVC}{\ProblemName{Partial Vertex Cover}}
\newcommand{\probPDS}{\ProblemName{Partial Dominating Set}}
\newcommand{\probPrDS}{\ProblemName{Partial $r$-Dominating Set}}
\newcommand{\probFVS}{\ProblemName{Feedback Vertex Set}}
\newcommand{\probIFVS}{\ProblemName{Independent Feedback Vertex Set}}
\newcommand{\probCycPacking}{\ProblemName{Cycle Packing}}
\newcommand{\probPlFVS}{\ProblemName{Planar Feedback Vertex Set}}
\newcommand{\probIS}{\ProblemName{Independent Set}}
\newcommand{\probWIS}{\ProblemName{Weighted Independent Set}}
\newcommand{\probMCIS}{\ProblemName{Multicolored Independent Set}}
\newcommand{\probDS}{\ProblemName{Dominating Set}}
\newcommand{\probrDS}{\ProblemName{$r$-Dominating Set}}
\newcommand{\probrSC}{\ProblemName{$r$-Scattered Set}}
%\newcommand{\probMDS}{\ProblemName{Minimum Dominating Set}}
\newcommand{\probPlDS}{\ProblemName{Planar Dominating Set}}
\newcommand{\probCDS}{\ProblemName{Connected Dominating Set}}
\newcommand{\probDST}{\ProblemName{Dominating Set on Tournaments}}
\newcommand{\probClique}{\ProblemName{Clique}}
\newcommand{\probMC}{\ProblemName{Multicolored Clique}}
\newcommand{\probPClique}{\ProblemName{Partitioned Clique}}
\newcommand{\probqSC}{\ProblemName{$q$-Set Cover}}
\newcommand{\probSC}{\ProblemName{Set Cover}}
\newcommand{\probDSP}{\ProblemName{Dominating Set with Pattern}}
%\newcommand{\probOCT}{\ProblemName{Odd Cycle Transversal}}
%\newcommand{\probEB}{\ProblemName{Edge Bipartization}}
\newcommand{\probHam}{\ProblemName{Hamiltonian Cycle}}
\newcommand{\probPlHam}{\ProblemName{Planar Hamiltonian Cycle}}
\newcommand{\probHamP}{\ProblemName{Hamiltonian Path}}
\newcommand{\probKPath}{\ProblemName{Longest Path}}
\newcommand{\probWKPath}{\ProblemName{Weighted Longest Path}}
\newcommand{\probthreeSAT}{\ProblemName{$3$-SAT}}
\newcommand{\probqSAT}{\ProblemName{$q$-SAT}}
\newcommand{\probcnfSAT}{\ProblemName{CNF-SAT}}
\newcommand{\probthreeCol}{\ProblemName{$3$-Coloring}}
\newcommand{\probqCol}{\ProblemName{$q$-Coloring}}
\newcommand{\probListColoring}{\ProblemName{List Coloring}}
\newcommand{\probOddSet}{\ProblemName{Odd Set}}
\newcommand{\probTuring}{\ProblemName{Short Turing Machine Acceptance}}
\newcommand{\probSI}{\ProblemName{Subgraph Isomorphism}}
\newcommand{\probGI}{\ProblemName{Graph Isomorphism}}
\newcommand{\probWCS}{\ProblemName{Weighted Circuit Satisfiability}}
\newcommand{\probClosestString}{\ProblemName{Closest String}}
\newcommand{\probClosestSubstring}{\ProblemName{Closest Substring}}
\newcommand{\probGridTiling}{\ProblemName{Grid Tiling}}
\newcommand{\probGridTilingLeq}{\ProblemName{Grid Tiling with~$\le$}}
\newcommand{\probUnitDisk}{\ProblemName{Unit Disk Independent Set}}
\newcommand{\probEMWay}{\ProblemName{Edge Multiway Cut}}
\newcommand{\probEDS}{\ProblemName{Edge Dominating Set}}
\newcommand{\probEMWaySets}{\ProblemName{Edge Multiway Cut for Sets}}
\newcommand{\probDirEMWay}{\ProblemName{Directed Edge Multiway Cut}}
\newcommand{\probEMCut}{\ProblemName{Edge Multicut}}
\newcommand{\probMulticut}{\ProblemName{Multicut}}
\newcommand{\probDirEMCut}{\ProblemName{Directed Edge Multicut}}
\newcommand{\probSkewEMCut}{\ProblemName{Skew Edge Multicut}}
\newcommand{\probDFVS}{\ProblemName{Directed Feedback Vertex Set}}
\newcommand{\probDFAS}{\ProblemName{Directed Feedback Arc Set}}
\newcommand{\probDFASC}{\ProblemName{Directed Feedback Arc Set Compression}}
\newcommand{\probPartpq}{\ProblemName{$(p,q)$-Partition}}
\newcommand{\probClusterpq}{\ProblemName{$(p,q)$-Cluster}}
\newcommand{\probSatellite}{\ProblemName{Satellite Problem}}
\newcommand{\probTw}{\ProblemName{Treewidth}}
\newcommand{\probPerfSetMatch}{\ProblemName{Perfect $d$-Set Matching}}
\newcommand{\probHS}{\ProblemName{Hitting Set}}
\newcommand{\probdHS}{\ProblemName{$d$-Hitting Set}}
\newcommand{\probEdHS}{\ProblemName{E$d$-Hitting Set}}
\newcommand{\probSetSplit}{\ProblemName{Set Splitting}}
\newcommand{\probSteiner}{\ProblemName{Steiner Tree}}
\newcommand{\probSteinerF}{\ProblemName{Steiner Forest}}
\newcommand{\probMotif}{\ProblemName{Graph Motif}}
\newcommand{\probColorfulMotif}{\ProblemName{Colorful Graph Motif}}
\newcommand{\probRBDSlong}{\ProblemName{Red-Blue Dominating Set}}
\newcommand{\probRBDS}{\ProblemNameX{RBDS}{Red-Blue Dominating Set}}
\newcommand{\probCRBDSlong}{\ProblemName{Colored Red-Blue Dominating Set}}
\newcommand{\probCRBDS}{\ProblemNameX{Col-RBDS}{Colored Red-Blue Dominating Set}}
\newcommand{\probCVC}{\ProblemName{Connected Vertex Cover}}
\newcommand{\probCFVS}{\ProblemName{Connected Feedback Vertex Set}}
\newcommand{\probCBullHit}{\ProblemName{Connected Bull Hitting}}
\newcommand{\probSetPacking}{\ProblemName{Set Packing}}
\newcommand{\probDisFactors}{\ProblemName{Disjoint Factors}}
\newcommand{\probDisPaths}{\ProblemName{Vertex Disjoint Paths}}
\newcommand{\probChromatic}{\ProblemName{Chromatic Number}}
\newcommand{\probECC}{\ProblemName{Edge Clique Cover}}
\newcommand{\probSubsetSum}{\ProblemName{Subset Sum}}
\newcommand{\probKnapsack}{\ProblemName{Knapsack}}
\newcommand{\probWayCut}{\ProblemName{$s$-Way Cut}}
\newcommand{\probEulerian}{\ProblemName{Eulerian  Deletion}}
\newcommand{\probBisec}{\ProblemName{Minimum Bisection}}
\newcommand{\probMaxBisec}{\ProblemName{Maximum Bisection}}


==> Saket/useless <==
\section{OCT in $H$-minor-free graphs}

Before describing our algorithm, we first introduce a generalization of the OCT problem, called \textit{constrained OCT}.

\begin{definition}
For a graph $G = (V,E)$ and a triple $(V_0,V_1,V_2)$ of subsets of $V$, we say an odd cycle transversal $V_\mathsf{oct}$ of $G$ is $(V_0,V_1,V_2)$-\textbf{compatible} if \textbf{(i)} $V_0 \subseteq V_\mathsf{oct}$ and \textbf{(ii)} $V_1 \backslash V_\mathsf{oct}$ and $V_2 \backslash V_\mathsf{oct}$ belong to different parts in the bipartite graph $G-V_\mathsf{oct}$.
\end{definition}
\begin{definition}[constrained OCT]
The \textbf{constrained OCT} problem is a parameterized problem in which each instance is a 5-tuple $(G,V_0,V_1,V_2,k)$ where $G$ is a graph, $V_0,V_1,V_2$ are three disjoint subsets of $V(G)$, and $k \in \mathbb{N}$ is the parameter, and the goal is to decide whether $G$ has an odd cycle transversal $V_\mathsf{oct}$ of size at most $k$ that $(V_0,V_1,V_2)$-compatible.
%\textbf{(i)} $V_0 \subseteq V_\mathsf{oct}$, $V_1 \subseteq I_1$, $V_2 \subseteq I_2$, \\
%\textbf{(ii)} $I_1$ and $I_2$ are independent sets in $G$, \\
%\textbf{(iii)} $|V_\mathsf{oct}| \leq k$.
\end{definition}

%Our main technical contribution is the following lemma, which plays an important role in our OCT algorithm for $H$-minor-free graphs.

%The proof of Lemma~\ref{lem-structure} will be given in Section~\ref{sec-proofstr}.
%Before this, let us first describe our OCT algorithm, assuming Lemma~\ref{lem-structure} holds.
Our OCT algorithm is obtained by (nontrivially) combining the ideas of Robertson-Seymour decomposition, recursive understanding, Baker's technique, and a technical lemma we establish about the structure of a graph that admits a good star decomposition (Lemma~\ref{lem-structure}).
Let $G$ be the input graph, which is $H$-minor-free.
Let $h > 0$ be the constant in Lemma~\ref{lem-rsdecomp} and $h'$ be the smallest integer that is larger than $|V(\mathsf{rep}(\mathcal{C}))|$ for any equivalence class $\mathcal{C}$ of $\equiv_\mathsf{oct}$ in $\mathcal{F}_{\subseteq [h]}$.

\paragraph{High-level framework.}
Algorithm~\ref{alg-OCT} presents the high-level framework of our algorithm.
The algorithm consists of an initialization step (Line~1), the main loop (Line~2-12), and a finalization step (Line~13).
In the initialization step, we compute an $(h,h')$-good tree decomposition $(T,\beta)$ for $G$ with adhesion size at most $h$ (together with the almost-embeddable structure of the torso of each internal node of $T$).
To this end, we first compute the Robertson-Seymour decomposition $(T_0,\beta)$ for $G$ (Lemma~\ref{lem-rsdecomp}), which has adhersion size at most $h$ and $h$-almost-embeddable torsos.
Then for each leaf $t \in T_0$, we add to $t$ a child $t'$ with bag $\beta(t') = \emptyset$; let $T$ be the resulting tree.
It is clear that $(T,\beta)$ is a tree decomposition of $G$ with adhesion size at most $h$.
Note that each leaf of $T$ has an empty bag and each internal node of $T$ is a node of $T_0$ (hence its torso is $h$-almost-embeddable).
So $(T,\beta)$ is $(h,0)$-good and thus an $(h,h')$-good.

The main loop (Line~2-12) is the heart of our algorithm.
Roughly speaking, during the loop, what we do is to iteratively \textit{simplify} the problem instance $(G,k)$.
That is, in each iteration, we generate a new instance $(G,k)$ from the old one such that the new instance is a YES-instance iff the old one is.
Meanwhile, we maintain the tree decomposition $(T,\beta)$ to guarantee that it is always an $(h,h')$-good tree decomposition of the current graph $G$ with adhesion size $h$.
A detailed discussion of the main loop will be given shortly.
Before this, we first discuss when the loop terminates and what we do in the finalization step.

We terminate the main loop when the problem instance $(G,k)$ becomes ``sufficiently simple'' in the sense that $|T| = 1$, i.e., the tree $T$ has only a root node (Line~2).
At this point, we reach the finalization step (Line~13), which simply solves the instance $(G,k)$ by \textit{brute-force}.
Why are we able to use brute-force when $|T| = 1$?
As mentioned before, $(T,\beta)$ is always an $(h,h')$-good tree decomposition of $G$.
When $|T|=1$, the bag $\beta(t)$ of the only node $t \in T$ is of size at most $h'$, because $t$ is a leaf and $(T,\beta)$ is $(h,h')$-good.
It follows that $G$ consists of a subgraph $G_0$ with $|V(G_0)| \leq h'$ and some isolated vertices.
Therefore, $(G,k)$ is a YES-instance iff $(G_0,k)$ is.
Since $|V(G_0)| \leq h'$, the instance $(G_0,k)$ can be solved in constant time by brute-force.

\begin{algorithm}[h]
    \caption{\textsc{OddCycleTransversal}$(G,k)$}
	\begin{algorithmic}[1]
        \State Compute an $(h,h')$-good tree decomposition $(T,\beta)$ of $G$ with adheresion size at most $h$
        %\State \textsc{Contract}$((T,\beta),h')$
        \While{$|T| \geq 2$}
            \State $t \leftarrow$ an internal node of $T$ whose children are all leaves
            %\State $X \leftarrow \gamma(t)$ and $B \leftarrow \sigma(t)$
            \State $\mathcal{I}_\mathsf{yes} \leftarrow \emptyset$
            \For{all $V_0,V_1,V_2 \subseteq \sigma(t)$ and all $l \in [k+h]$}
                \State Solve the constrained OCT instance $(G[\gamma(t)],V_0,V_1,V_2,l)$
                \If{$(G[\gamma(t)],V_0,V_1,V_2,l)$ is a YES-instance}
                    \State $\mathcal{I}_\mathsf{yes} \leftarrow \mathcal{I}_\mathsf{yes} \cup \{(G[\gamma(t)],V_0,V_1,V_2,l)\}$
                \EndIf
            \EndFor
            \If{$(G[\gamma(t)],\emptyset,\emptyset,\emptyset,k) \notin \mathcal{I}_\mathsf{yes}$}
                \textbf{return} NO
            \EndIf
            %\State $\lambda \leftarrow$ an arbitrary bijection from $\sigma(t)$ to $[|\sigma(t)|]$
            %\State view both $G[\gamma(t)]$ and $G[\gamma'(t)]$ as boundaried graphs in $\mathcal{F}_{[|\sigma(t)|]}$
            \State $(G^*,c) \leftarrow$ \textsc{Representative}$(G[\gamma(t)],\mathcal{I}_\mathsf{yes})$
            \State $G \leftarrow G^* \oplus G[\gamma'(t)]$ and $k \leftarrow k-c$
            \State Modify $(T,\beta)$ by replacing the subtree $T_t$ with a single node $t^*$ with $\beta(t^*) = V(G^*)$
            %\State \textsc{Contract}$((T,\beta),h')$
        \EndWhile
        \State Solve the instance $(G,k)$ by brute-force
        %\nolinenumbers
	\end{algorithmic}
	\label{alg-OCT}
\end{algorithm}

In what follows, we discuss the main loop in detail.
In each iteration of the loop, we first pick an (arbitrary) internal node $t \in T$ whose children are all leaves (Line~3).
Note that the subtree $T_t$ is a star.
Consider the induced subgraph $G[\gamma(t)]$.
Fix a bijection $\lambda: \sigma(t) \rightarrow [|\sigma(t)|]$.
We can view $G[\gamma(t)]$ as a boundaried graph in $\mathcal{F}_{[|\sigma(t)|]}$ with boundary $\sigma(t)$ and labeling $\lambda$.
%Similarly, the labeling $\lambda$ also makes $G[\gamma'(t)]$ a boundaried graph in $\mathcal{F}_{[|\sigma(t)|]}$, and we have $G = G[\gamma(t)] \oplus G[\gamma'(t)]$.
Our goal in this iteration is to compute a progressive representative of the equivalent class of $\equiv_\mathsf{oct}$ containing $G[\gamma(t)]$.
To this end, the critical step is to solve a set of constrained OCT instances on $G[\gamma(t)]$ (Line~5-8).
Specifically, we solve the instances $(G[\gamma(t)],V_0,V_1,V_2,l)$ for all $V_0,V_1,V_2 \subseteq \sigma(t)$ and all $l \in [k+h]$.
This is the most technical part of our algorithm, and the main idea is to exploit the fact that $G[\gamma(t)]$ has a $(h,h')$-good \textit{star} decomposition, which is $(T_t,\beta)$.
We shall establish a structural lemma (Lemma~\ref{lem-structure}) for graphs that admit a good star decomposition, which then allows us to apply Baker's technique and dynamic programming on tree decomposition to solve the problem.
After the constrained OCT instances are solved, we then include the YES-instances (Line~8) in $\mathcal{I}_\mathsf{yes}$.
If $(G[\gamma(t)],\emptyset,\emptyset,\emptyset,k) \notin \mathcal{I}_\mathsf{yes}$, then we can immediately conclude that $(G,k)$ is a NO-instance (Line~9), because $(G[\gamma(t)],k)$ is a NO-instance.
Otherwise, we use the information of $\mathcal{I}_\mathsf{yes}$ to compute a progressive representative of the equivalent class of $\equiv_\mathsf{oct}$ containing $G[\gamma(t)]$ and the corresponding transposition (Line~10).
Specifically, the sub-routine \textsc{Representative} takes $G[\gamma(t)]$ and $\mathcal{I}_\mathsf{yes}$ as input, and output a pair $(G^*,c)$ where $G^*$ is a progressive representative of the equivalent class containing $G[\gamma(t)]$ and $c \in \mathbb{Z}^+$ is the transposition from $G[\gamma(t)]$ to $G'$.
Note that $G = G[\gamma(t)] \oplus G[\gamma'(t)]$, if we regard $G[\gamma'(t)]$ as a boundaried graph with boundary $\sigma(t)$ and labeling $\lambda$.
Thus, by the definition of a progressive representative, we know that $(G,k)$ is a YES-instance of OCT iff $(G^* \oplus G[\gamma'(t)],k-c)$ is.
We then replace $(G,k)$ with $(G^* \oplus G[\gamma'(t)],k-c)$ (Line~11).
After this, we modify the tree decomposition $(T,\beta)$ by replacing the subtree $T_t$ with a single node $t^*$ with $\beta(t^*) = V(G^*)$ (Line~12).
It is easy to see that after the modification, $(T,\beta)$ is a tree decomposition of the new $G$, i.e., $G^* \oplus G[\gamma'(t)]$, which is still $(h,h')$-good and with adhesion size at most $h$.
Furthermore, $|T|$ strictly decreases after the modification.
Therefore, the loop will terminate in at most $m$ iterations, where $m$ is the initial size of $T$.
This directly implies the correctness of our algorithm.
Next, we discuss the only two missing pieces of our algorithm, which are \textbf{(1)} how to solve the instances on $G[\gamma(t)]$ (Line~6) and \textbf{(2)} how to compute the progressive representative $G^*$ and the transposition $c$ (Line~10).

\paragraph{Solving the instances on $G[\gamma(t)]$.}
Consider a constrained OCT instance $(G[\gamma(t)],V_0,V_1,V_2,l)$ where $V_0,V_1,V_2 \subseteq \sigma(t)$ and $l \in [k+h]$.
We want to test if there exists a $(V_0,V_1,V_2)$-compatible OCT of $G[\gamma(t)]$ of size at most $l$.
If $l < |V_0|$, then $(G[\gamma(t)],V_0,V_1,V_2,l)$ is clearly a NO-instance.
So assume $l \geq |V_0|$.
First, we notice that using Lemma~\ref{lem-candidate}, we are able to compute a small relevant set for the instance.
\begin{corollary} \label{cor-candidate}
We can compute in $|\gamma(t)|^{O(1)}$ time a set $S \subseteq \gamma(t)$ of size $l^{O(1)}$ such that with probability at least $1-1/2^{|\gamma(t)|}$, $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size $l$ iff $G$ has a $(V_0,V_1,V_2)$-compatible OCT of size $l$ that is contained in $S$.
\end{corollary}
\begin{proof}
Let $G'$ be the graph obtained from $G[\gamma(t)] - V_0$ by adding edges $(u,v)$ for all $u \in V_1 \backslash V_0$ and $v \in V_2 \backslash V_0$.
One can easily verify that a subset $U \subseteq V(G')$ is an OCT of $G'$ iff $U \cup V_0$ is a $(V_0,V_1,V_2)$-compatible OCT of $G[\gamma(t)]$.
Furthermore, every $(V_0,V_1,V_2)$-compatible OCT of $G[\gamma(t)]$ can be written as $U \cup V_0$ where $U$ is an OCT of $G'$.
In other words, the map $U \mapsto U \cup V_0$ gives a one-to-one correspondence between the OCTs of $G'$ and the $(V_0,V_1,V_2)$-compatible OCTs of $G[\gamma(t)]$.
Therefore, if we use the algorithm of Lemma~\ref{lem-candidate} to compute a set $S' \subseteq V(G')$ of size $(l-|V_0|)^{O(1)}$ such that $G'$ has an OCT of size $l-|V_0|$ iff $G'$ has an OCT of size $l-|V_0|$ that is contained in $S'$, then the set $S = S' \cup V_0$ satisfies the property that $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size $l$ iff $G$ has a $(V_0,V_1,V_2)$-compatible OCT of size $l$ that is contained in $S$.
\end{proof}

Let $S \subseteq \gamma(t)$ be the set in the above corollary.
As mentioned before, we shall exploit the fact that $G[\gamma(t)]$ has an $(h,h')$-good star decomposition with adhesion size $h$.
To this end, we establish the following technical lemma, whose proof is deferred to Section~\ref{sec-proofstr}.

\begin{lemma} \label{lem-structure}
Let $G$ be a graph admitting a $(c,c')$-good star decomposition with adhesion size $c''$ for some constants $c,c',c''$.
Then for any $p \in [n]$, there are $Z_1,\dots,Z_p \subseteq V(G)$ satisfying the following. \\
\textbf{(i)} Each vertex $v \in V(G)$ is contained in at most $c''$ sets in $\{Z_1,\dots,Z_p\}$. \\
\textbf{(ii)} For any $i \in [p]$ and $V' \subseteq Z_i$, $\mathbf{tw}(G/(Z_i-V')) = O(p+|V'|)$, where the constant hidden in the big-$O$ notation depends on $c,c',c''$. \\
%one can compute in $|V(G)|^{O(1)}$ time a tree decomposition of $G \backslash V'$ in which each bag contains $O(p)$ vertices in $V(G) \backslash V_i$ and intersects $O(p')$ connected component of $G[V_i \backslash V']$ where $p' = |V'|$. \\
Furthermore, if the good star decomposition of $G$ (and the almost-embeddable structure of the torso of the central bag) is given, then the above sets $Z_1,\dots,Z_p$ can be computed in $|V(G)|^{O(1)}$ time.
\end{lemma}

We apply the above lemma with $G = G[\gamma(t)]$ and $p = \lfloor\sqrt{l}\rfloor$, and obtain the sets $Z_1,\dots,Z_p \subseteq V(G[\gamma(t)]) = \gamma(t)$.
We claim that $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size at most $l$ iff for some $i \in [p]$ and $V' \subseteq Z_i \cap S$ with $|V'| \leq hl/p$, $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size at most $l$ that is \textit{disjoint} with $Z_i - V'$.
The ``if'' part is obvious.
To see the ``only if'' part, assume $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size at most $l$.
Then it has a $(V_0,V_1,V_2)$-compatible OCT $V_\mathsf{oct} \subseteq S$ of size at most $l$ by Corollary~\ref{cor-candidate}.
By the property \textbf{(i)} in Lemma~\ref{lem-structure}, each vertex $v \in \gamma(t)$ is contained in at most $h$ sets in $\{Z_1,\dots,Z_p\}$.
Therefore, we have $|V_\mathsf{oct} \cap Z_i| \leq hl/p$ for some $i \in [p]$.
Set $V' = V_\mathsf{oct} \cap Z_i$.
Since $V_\mathsf{oct} \subseteq S$, we have $V' \subseteq Z_i \cap S$.
Also, we have $V_\mathsf{oct} \cap (Z_i - V') = \emptyset$, which implies our claim.
With this claim, it now suffices to test, for every pair $(i,V')$ where $i \in [p]$ and $V' \subseteq Z_i \cap S$ is of size at most $hl/p$, whether $G[\gamma(t)]$ has a $(V_0,V_1,V_2)$-compatible OCT of size at most $l$ that is disjoint with $Z_i - V'$.

\begin{lemma}
Let $G$ be a graph, $Z \subseteq V(G)$, and $w = \mathbf{tw}(G/Z)$.
Given any $V_0,V_1,V_2 \subseteq V(G)$, one can compute in $w^{O(w)} \cdot |V(G)|^{O(1)}$ time a minimum-sized $(V_0,V_1,V_2)$-compatible OCT of $G$ that is contained in $V(G) - Z$ (or decide the non-existence of such an OCT).
\end{lemma}

\paragraph{Computing a progressive representative.}

\subsection{Proof of Lemma~\ref{lem-structure}} \label{sec-proofstr}

\section{OCT in unit-disk graphs}

\begin{lemma} \label{lem-structure1}
Given the representation of an $n$-vertex unit-disk graph $G$ and an integer $p \in [n]$, one can compute in $n^{O(1)}$ time a partition $\{V_1,\dots,V_p\}$ of $V(G)$ and a clique tree decomposition of $G/V_i$ with width $O(p)$ for each $i \in [p]$.
\end{lemma}

\subsection{Proof of Lemma~\ref{lem-structure1}}

Let $\langle \mathcal{D},k \rangle$ be the input of the problem, where $\mathcal{D}$ is a set of $n$ disks in the plane and $k$ is the parameter.
Let $G_\mathcal{D} = (\mathcal{D},E)$ be the unit-disk graph defined by $\mathcal{D}$.

\paragraph{The layering procedure.}
We compute a layering $\ell: \mathcal{D} \rightarrow \mathbb{N}$ of the disks as follows.
First, we build a grid $\varGamma$ consisting of squares with side-length $\frac{1}{2}$.
For a unit disk $D$, we use the notation $\Box_D$ to denote the cell of $\varGamma$ that contains the center of $D$.
Furthermore, for a cell $\Box$ of $\varGamma$ and a set $\mathcal{X}$ of unit disks, we use the notation $\mathcal{X}(\Box)$ to denote the subset of unit disks in $\mathcal{X}$ whose centers are in $\Box$.
Then our layering procedure is the following.

\begin{algorithm}[h]
    \caption{\textsc{Layering}$(\mathcal{D})$ \Comment{Output a layering $\ell: \mathcal{D} \rightarrow \mathbb{N}$}}
	\begin{algorithmic}[1]
        \State $t \leftarrow 0$
        \While{$\mathcal{D} \neq \emptyset$}
            \State $t \leftarrow t + 1$
            \State $\mathcal{D}_\mathsf{out} \leftarrow \{D \in \mathcal{D}: D \text{ is exposed on the outer boundary of } \bigcup_{D \in \mathcal{D}} D\}$
            \State $\mathcal{L} \leftarrow \bigcup_{D \in \mathcal{D}_\mathsf{out}} \mathcal{D}(\Box_D)$
            \State $\ell(D) \leftarrow \lceil t/100 \rceil$ for all $D \in \mathcal{L}$
            \State $\mathcal{D} \leftarrow \mathcal{D} \backslash \mathcal{L}$
        \EndWhile
        \State \textbf{return} $\ell$
	\end{algorithmic}
	\label{alg-layering}
\end{algorithm}

\paragraph{Basic properties of the layering.}
Let $\ell: \mathcal{D} \rightarrow \mathbb{N}$ be the layering of $\mathcal{D}$ obtained using the above algorithm.
For convenience, we write $\mathcal{L}_i = \ell^{-1}(\{i\})$ and call it \textit{the $i$-th layer}.
Suppose there are in total $m$ layers.
We define $\mathcal{L}_{>i} = \bigcup_{j=i+1}^m \mathcal{L}_j$ and $\mathcal{L}_{[i',i]} = \bigcup_{j=i'}^i \mathcal{L}_j$.
We now establish some basic properties of our layering.
\begin{lemma}
For any $D,D' \in \mathcal{D}$ such that $D \cap D' \neq \emptyset$, we have $|\ell(D) - \ell(D')| \leq 1$.
\end{lemma}

\begin{lemma}
Let $C$ be a connected component of $G[\mathcal{L}_{>i}]$.
Then $N(C) \cap \mathcal{L}_i$ lies in a connected component of $G[\mathcal{L}_i]$.
\end{lemma}

\begin{lemma}
The induced subgraph $G[\mathcal{L}_{[i',i]}]$ has tree width $O(s)$ after contracting the vertices in the same cell of $\varGamma$ into a single vertex, where $s = i'-i+1$.
\end{lemma}

\begin{fact}
Let $G = (V,E)$ be a connected unit-disk graph.
Then for any $V' \subseteq V$ of size $d$, the induced subgraph $G [V \backslash V']$ consists of $O(d)$ connected components.
\end{fact}

==> useless <==
We claim that the interior of $E_S \backslash (\bigcup_{u \in I^*} D_u)$ is homeomorphic to an open disk.
Because $E_S$ is the intersection of the disks in $\mathcal{D}_S$, it is topologically homeomorphic to a (closed) disk.
By Observation~\ref{obs-S*I*pro2}, each disk $D_u$ for $u \in I^*$ is not contained in $\bigcup_{w \in \{v\} \cup S^*} D_w$ and in particular is not contained in $\bigcup_{w \in \{v\} \cup \mathcal{D}_S} D_w$.
Therefore, the boundary of $D_u$ intersects the boundary of $E_S$ at most twice by Lemma~\ref{lem-inttwice}.
For convenience, suppose $I^* = \{u_1,\dots,u_m\}$.
We show by induction on $r$ that the interior of $E_S \backslash (\bigcup_{i=1}^r D_{u_i})$ is homeomorphic to an open disk for all $r \in [m]$.
When $r = 0$, $E_S \backslash (\bigcup_{i=1}^r D_{u_i}) = E_S$ and the statement holds as $E_S$ is homeomorphic to an open disk.
Assume the interior of $E_S \backslash (\bigcup_{i=1}^{r-1} D_{u_i})$ is homeomorphic to an open disk and we show the interior $E_S \backslash (\bigcup_{i=1}^r D_{u_i})$ is also homemorphic to an open disk.
Let $C$ be the closure of $E_S \backslash (\bigcup_{i=1}^{r-1} D_{u_i})$, which is homeomorphic to a (closed) disk.
Each arc on the boundary of $C$ is a portion of the boundary of $E_S$ or the boundary of $D_{u_i}$ for some $i \leq r-1$.
As the boundary of $D_{u_r}$ intersects the boundary of $E_S$ at most twice and does not intersect the boundaries of $D_{u_1},\dots,D_{u_{r-1}}$, it can intersect the boundary of $C$ at most twice.
Note that $D_{u_r} \nsubseteq C$ since $D_{u_r} \nsubseteq \bigcup_{w \in \{v\} \cup S^*} D_w$.
Therefore, if the boundary of $D_{u_r}$ and the boundary of $C$ do not intersect or intersect only once, $D_{u_r}$ is disjoint from the interior of $C$, i.e., the interior of $E_S \backslash (\bigcup_{i=1}^{r-1} D_{u_i})$.
In this case, the interior of $E_S \backslash (\bigcup_{i=1}^r D_{u_i})$ is just the interior of $E_S \backslash (\bigcup_{i=1}^{r-1} D_{u_i})$ and we are done.
So suppose the boundary of $D_{u_r}$ intersects the boundary of $C$ twice.
By Jordan curve theorem, the portion of the boundary of $D_{u_r}$ contained in $C$ partitions $C$ into two parts, one inside $D_{u_r}$ and one outside, and the interior of each part is homeomorphic to an open disk.
The interior of the part outside $D_{u_r}$ is just the interior of $E_S \backslash (\bigcup_{i=1}^r D_{u_i})$, which implies the latter is homeomorphic to an open disk.
This induction argument shows the interior of $E_S \backslash (\bigcup_{u \in I^*} D_u) = E_S \backslash (\bigcup_{i=1}^m D_{u_i})$ is homeomorphic to an open disk.

------------------------------------

Define a sequence $\delta_0,\delta_1,\dots,\delta_{|S^*|}$ of numbers as $\delta_0 = 1$ and $\delta_d = (2 \delta_{d-1} + 3) \cdot 5|S^*|$ for $d \geq 1$.
Since $|S^*| = O_\varepsilon(1)$ by Observation~\ref{obs-S*I*pro1}, $\delta_d = O_\varepsilon(1)$ for all $d \leq |S^*|$.
We show that $\mathsf{rad}(A_{\mathcal{D}'}[E_S]) \leq \delta_d$ for all $S \subseteq S^*$, where $d = |S^* \backslash S|$.
Note that when $S = \emptyset$, this implies $\mathsf{rad}(A_{\mathcal{D}'}[D_v]) = O_\varepsilon(1)$, as $E_\emptyset = D_v$.
We apply induction on $d$.
%Write $\delta_d = 5^d (|S^*|+1)^d$ for convenience.
For $d=0$, we have $S = S^*$ and we want $\mathsf{rad}(A_{\mathcal{D}'}[E_{S^*}]) \leq \delta_0 = 1$.
Since $\mathcal{D}' = \mathcal{D}_{S^*}^+$, Observation~\ref{obs-star} implies $A_{\mathcal{D}'}[E_{S^*}]$ is a star (or an empty graph if $E_{S^*} = \emptyset$) and thus $\mathsf{rad}(A_{\mathcal{D}'}[E_{S^*}]) \leq 1$.
Assume the statement holds for $d-1$ and we prove it also holds for $d$.
Let $S \subseteq S^*$ such that $|S^* \backslash S| = d$.
We want $\mathsf{rad}(A_{\mathcal{D}'}[E_S]) \leq \delta_d$.
If $E_S = \emptyset$, we are done, as in this case $A_{\mathcal{D}'}[E_S]$ is an empty graph.
So suppose $E_S \neq \emptyset$.
Let $\mathcal{F}$ (resp., $\mathcal{F}_0$) be the set of arrangement faces of $\mathcal{D}'$ (resp., $\mathcal{D}_S^+$) contained in $E_S$.
Because $\mathcal{D}_S^+ \subseteq \mathcal{D}'$, each face in $\mathcal{F}$ is contained in some face in $\mathcal{F}_0$.
It can happen that one face $F \in \mathcal{F}$ is also a face in $\mathcal{F}_0$; in this case, we call $F$ a \textit{preserved} face.
We say a face $F \in \mathcal{F}$ is \textit{witnessed} by a vertex $u \in S^* \backslash S$ if $F$ is contained in $D_u$ or $F$ is adjacent to a face that is contained in $D_u$ (equivalently, one arc of the boundary of $F$ is contributed by $D_u$).
Note that a face can be witnessed by multiple vertices in $S^* \backslash S$.
\begin{observation}
A face $F \in \mathcal{F}$ not witnessed by any vertex in $S^* \backslash S$ is a preserved face.
\end{observation}
\begin{proof}
If $F \in \mathcal{F}$ is not witnessed by any vertex in $S^* \backslash S$, then all arcs of the boundary of $F$ are contributed by the disks in $\mathcal{D'} \backslash \{D_u: u \in S^* \backslash S\} = \mathcal{D}_S^+$, and hence $F$ is also a face of the arrangement of $\mathcal{D}_S^+$ (i.e., $F \in \mathcal{F}_0$), which implies $F$ is a preserved face.
\end{proof}

%\begin{observation}
%All but one preserved faces in $\mathcal{F}$ are degree-1 vertices in $A_{\mathcal{D}'}[E_S]$.
%\end{observation}
%\begin{proof}
%By Observation~\ref{obs-star}, $A_{\mathcal{D}_S^+}[E_S]$ is a star and thus all faces in $\mathcal{F}_0$ except the one corresponding to the center of the star are pairwise
%\end{proof}

\begin{observation} \label{obs-witness}
For two faces $F,F' \in \mathcal{F}$ witnessed by the same vertex $u \in S^* \backslash S$, the shortest-path distance between $F$ and $F'$ in the graph $A_{\mathcal{D}'}[E_S]$ is $2 \delta_{d-1} + 2$.
\end{observation}
\begin{proof}
We define a face $P \in \mathcal{F}$ for $F$ as follows.
If $F \subseteq D_u$, we set $P = F$.
If $F \nsubseteq D_u$, then one arc $\sigma$ of the boundary of $F$ must be contributed by $D_u$, as $F$ is witnessed by $u$.
In this case, we set $P$ to be the face sharing the arc $\sigma$ with $F$, which is contained in $D_u$ (as $F \nsubseteq D_u$).
Note that $P \in \mathcal{F}$.
Indeed, since $F \subseteq E_S$ and the arc $\sigma$ is not on the boundary of $E_S$, we have $P \subseteq E_S$ and $P \in \mathcal{F}$.
%By our induction hypothesis, $\mathsf{rad}(A_{\mathcal{D}'}[E_{S \cup \{u\}}]) \leq \delta_{d-1}$ since $|S^* \backslash (S \cup \{u\})| = d-1$.
In the same way, we can define a face $P' \in \mathcal{F}$ for $F'$: if $F' \subseteq D_u$, we set $P' = F'$, otherwise we let $P'$ be the face sharing with $F'$ an arc contributed by $D_u$.
Now $P,P' \in \mathcal{F}$ and $P,P' \subseteq D_u$.
So $P$ and $P'$ are both vertices of $A_{\mathcal{D}'}[E_{S \cup \{u\}}]$.
By our induction hypothesis, $\mathsf{rad}(A_{\mathcal{D}'}[E_{S \cup \{u\}}]) \leq \delta_{d-1}$ since $|S^* \backslash (S \cup \{u\})| = d-1$.
Therefore, there is a path $\pi$ from $P$ to $P'$ in $A_{\mathcal{D}'}[E_{S \cup \{u\}}]$ of length at most $2 \delta_{d-1}$.
Clearly, $\pi$ is also a path in $A_{\mathcal{D}'}[E_S]$, as $A_{\mathcal{D}'}[E_{S \cup \{u\}}]$ is an induced subgraph of $A_{\mathcal{D}'}[E_S]$.
Finally, because $P$ is either $F$ or is adjacent to $F$ (resp., $P'$ is either $F'$ or is adjacent to $F'$), there exists a path from $F$ to $F'$ in $A_{\mathcal{D}'}[E_S]$ of length at most $2 \delta_{d-1}+2$.
\end{proof}

Now we are ready to show $\mathsf{rad}(A_{\mathcal{D}'}[E_S]) \leq \delta_d$.
To this end, consider a path $\pi = (F_0,F_1,\dots,F_r)$ in $A_{\mathcal{D}'}[E_S]$ and suppose $\pi$ is a shortest path from $F_0$ to $F_r$ in $A_{\mathcal{D}'}[E_S]$.
We claim $r \leq \delta_d$.
First observe that for every $u \in S^* \backslash S$, the number of faces in $\{F_1,\dots,F_r\}$ witnessed by $u$ is at most $2 \delta_{d-1} + 3$.
Indeed, if there are more than $2 \delta_{d-1} + 3$ faces in $\{F_1,\dots,F_r\}$ witnessed by $u$, then one can find two indices $i,j \in [r]$ such that $F_i$ and $F_j$ are witnessed by $u$ and $j-i \geq 2 \delta_{d-1} + 3$.
Observation~\ref{obs-witness} implies the shortest-path distance between $F_i$ and $F_j$ $A_{\mathcal{D}'}[E_S]$ is at most $2 \delta_{d-1} + 2$.
But the subpath $(F_i,\dots,F_j)$ of $\pi$ is of length at least $2 \delta_{d-1} + 3$, which contradicts the fact that $\pi$ is a shortest path in $A_{\mathcal{D}'}[E_S]$.
It follows that the number of faces in $\{F_1,\dots,F_r\}$ witnessed by any vertex in $S^* \backslash S$ is at most $(2 \delta_{d-1} + 3) \cdot |S^*|$.

Let $\mathcal{F}$ (resp., $\mathcal{F}'$) be the set of arrangement faces of $\mathcal{D}_S^+$ (resp., $\mathcal{D}'$) contained in $E_S$, i.e., vertices of $A_{\mathcal{D}_S^+}[E_S]$ (resp., $A_{\mathcal{D}'}[E_S]$).
Since $\mathcal{D}_S^+ \subseteq \mathcal{D}'$, every face in $\mathcal{F}'$ is contained in some face in $\mathcal{F}$.
More specifically, the faces in $\mathcal{F}'$ are obtained by subdividing the faces in $\mathcal{F}$ using the boundaries of the disks in $\mathcal{D}' \backslash \mathcal{D}_S^+ = \{D_u: u \in S^* \backslash S\}$.
It can happen that one face in $\mathcal{F}$ is also a face in $\mathcal{F}'$ (when the face is not cut by the boundary of any disk in $\mathcal{D}' \backslash \mathcal{D}_S^+$); in this case, we call it a \textit{preserved} face.
A face in $\mathcal{F}'$ is a \textit{new} face if it is not a preserved face.
Note that at least one face in $\mathcal{F}'$ is new, for otherwise $\mathcal{F}' = \mathcal{F}$ and $E_S$ does not intersect $D_u$ for any $u \in S^* \backslash S$, which contradicts the assumption that $S$ is not maximal in $\mathcal{S}$.
We prove the observation by first showing every new face in $\mathcal{F}'$ is within distance 1 from a face $F'  \in \mathcal{F}'$ with $S \subsetneq S_{F'}$ and showing that every preserved face is within distance 2 from a new face.
Here ``distance'' refers to the shortest-path distance in $A_{\mathcal{D}'}[D_v]$.
This directly implies any face in $\mathcal{F}'$ (in particular, the face $F$) is within distance 3 from some face $F' \in \mathcal{F}'$ with $S \subsetneq S_{F'}$.

Consider a new face $F_0 \in \mathcal{F}'$.
If $S \subsetneq S_{F_0}$, we simply set $F' = F_0$.
Otherwise, $S = S_{F_0}$.
Since $F_0$ is a new face, one arc $\sigma$ of the boundary of $F$ must be contributed by $D_u$ for some $u \in S^* \backslash S$\todo{I did not follow. Maybe a figure for this obs will be good}.
Then we simply let $F'$ be the face that shares the arc $\sigma$ with $F$.
Note that $S_{F'} = S \cup \{u\}$ and thus $S \subsetneq S_{F'}$.
The distance between $F$ and $F'$ is 1 as they share the arc $\sigma$.
Also, $F' \in \mathcal{F}'$ simply because $F_0 \in \mathcal{F}'$ and $\sigma$ is not on the boundary of $E_S$.
This shows every new face in $\mathcal{F}'$ is within distance 1 from a face $F' \in \mathcal{F}$ with $S \subsetneq S_{F'}$.

Next, consider a preserved face $F_0 \in \mathcal{F}'$.
By definition, $F_0 \in \mathcal{F}$, i.e., $F_0$ is a vertex of $A_{\mathcal{D}_S^+}[E_S]$.
%If $F_0$ is adjacent to a new face in $\mathcal{F}'$, we are done.
By Observation~\ref{obs-star}, $A_{\mathcal{D}_S^+}[E_S]$ is a star.
We distinguish two cases: $F_0$ is the center of the star $A_{\mathcal{D}_S^+}[E_S]$ or not.
If $F_0$ is the center, then $F_0$ is neighboring to all other vertices in $A_{\mathcal{D}_S^+}[E_S]$, and equivalently, adjacent to all other faces in $\mathcal{F}$.
As argued before, at least one face in $\mathcal{F}$ is not preserved in $\mathcal{F}'$.
Since $F_0$ is a preserved face and adjacent to all other faces in $\mathcal{F}$, there must be one face $F_1 \in \mathcal{F}$ adjacent to $F_0$ that is not preserved in $\mathcal{F}'$.
All faces in $\mathcal{F}'$ contained in $F_1$ are new faces, and at least one of them is adjacent to $F_0$ (as $F_1$ is adjacent to $F_0$).
So $F_0$ is within distance 1 from a new face in $\mathcal{F}'$.
If $F_0$ is not the center of $A_{\mathcal{D}_S^+}[E_S]$, let $F_1 \in \mathcal{F}$ be the center.
Then $F_0$ and $F_1$ are adjacent.
If $F_1$ is not preserved in $\mathcal{F}'$, then the above argument shows that $F_0$ is within distance 1 from a new face in $\mathcal{F}'$ that is contained in $F_1$.
If $F_1$ is preserved in $\mathcal{F}'$, then our discussion of the first case shows that $F_1$ is within distance 1 from a new face in $\mathcal{F}'$ and thus $F_0$ is within distance 2 from a new face in $\mathcal{F}'$.
Combining the two cases, we conclude that any preserved face in $\mathcal{F}'$ is within distance 2 from a new face in $\mathcal{F}'$.




So far we have shown how to prove Lemma~\ref{lem-reduction2} under the assumption that a realization $\mathcal{D}$ of $G_1$ is known.
So the only missing piece now is to make our reduction work without the assumption.
Note that the only place we use the realization $\mathcal{D}$ in Algorithm~\ref{alg-reduction2} is when we order the vertices of $G_1$ in line~1.
Here, we need the sorted sequence $(v_1,\dots,v_n)$ to satisfy $D_{v_1} \geq \cdots \geq D_{v_n}$, and this seems impossible if $\mathcal{D}$ is not given.
However, the property $D_{v_1} \geq \cdots \geq D_{v_n}$ is in fact only used for proving Observation~\ref{obs-nghbO1} and~\ref{obs-nghbnghb}.
Therefore, as long as the sequence $(v_1,\dots,v_n)$ satisfies Observation~\ref{obs-nghbO1} and~\ref{obs-nghbnghb} for all $i \in [n]$, the reduction of Algorithm~\ref{alg-reduction2} is correct (with the totally same analysis).
So it suffices to design an ordering procedure $\textsc{Order}(G_1)$ that can return a sequence $(v_1,\dots,v_n)$ satisfying Observation~\ref{obs-nghbO1} and~\ref{obs-nghbnghb}, and use it in line~1 of Algorithm~\ref{alg-reduction2}.
Clearly, this procedure should run in $n^{O(1)}$ time and only depends on $G_1$ itself.



\todo[inline]{The proofs of below two observations has considerable similarity with other two observations. We may avoid both together in first 10 pages}

%in line~1 of Algorithm~\ref{alg-reduction2} 

%Indeed, we have $S^-(v_i) \cap R_j = N_{G_2}(v_i) \cap R_j \cap \{v_{i+1},\dots,v_n\}$ by definition.
%If $S^-(v_i) \cap R_j \neq \emptyset$, then $R_j$ contains at least one vertex in $N_{G_2}(v_i) \cap \{v_{i+1},\dots,v_n\}$.
